Which Combination of Test Metrics Can Predict Success of a Software Project? A Case Study in a Year-Long Project Course

Testing plays an important role in securing the success of a software development project. Prior studies have demonstrated beneficial effects of applying acceptance testing within a Behavioural-Driven Development method. In this research, we investigate whether we can quantify the effects various types of testing have on functional suitability, i.e. the software conformance to users' functional expectations. We explore which combination of software testing (automated and manual, including acceptance testing) should be applied to ensure the expected functional requirements are met, as well as whether the lack of testing during a development iteration causes a significant increase of effort spent fixing the project later on. To answer those questions, we collected and analysed data from a year-long software engineering project course. We combined manual observations and statistical methods, namely Linear Mixed-Effects Modelling, to evaluate the effects of coverage metrics as well as time effort on passed stories over 5 Scrum sprints. The results suggest that a combination of a high code coverage for all of automated unit, acceptance, and manual testing has a significant impact on functional suitability. Similarly, but to a lower extent, front-end unit testing and manual testing can predict the success of a software delivery when taken independently. We observed a close-to-significant effect between low back-end testing and deferral (i.e. postponement) of user stories.

==> acm_legacy-do-not-edit/content.tex <==

\section{Introduction}
\label{sec:introduction}

Agile software development favours lighter upfront requirement analysis with shorter delivery cycles~\cite{Beck2000}. Among other practices embraced by the agile movement, continuous integration has improved software development and release processes \textit{``thanks specifically to a sharper focus on metrics and process standardization''}~\cite{Roche2013}. Furthermore, there has been a push to blur the lines between the developers who build a software product and the operators running a set of quality assurance checks and support clients, commonly referred to as DevOps~\cite{Stahl2017}. Developers are expected to contribute to quality assurance processes by automating the testing for the code they write. Within that method framework, automation is a crucial factor, including for (continuous) testing purposes~\cite{Lwakatare2015}. Therefore, technologies have emerged to test both units of code (\textit{e.g., JUnit, Jest}) and delivered features as requested by the user (\textit{i.e} user acceptance testing, e.g., Cucumber).

However, benefits of continuous integration can be lost when a development process exhibits some antipatterns such as the lack of automated testing, including in production-like environments~\cite{Zampetti2020}, which create software products of low quality. Code coverage metrics are a common way to ensure a software behaves as expected where batteries of automated tests are checking all possible execution paths of the software~\cite{Bertolino2007}. However, high coverage metrics are not always linked to good tests~\cite{Inozemtseva2014}, as confirmed by Bai \textit{et al.}'s survey with students who considered code coverage as the most important metric, but the same students tended to test only blue sky scenarios~\cite{Bai2021}. Therefore, in this work, we go beyond by analysing the testing effort from multiple viewpoints, i.e. unit, acceptance and manual testing on the one hand, and the overall testing effort in terms of lines of code and time spent testing on the other hand.

Our focus in this research is to empirically investigate the relationship between the testing behaviour of a team of junior developers and the external quality of the software produced during a year-long software engineering project. In other words, we investigate \textbf{to what extend a combination of metrics related to automated unit testing, automated user acceptance testing, manual testing and testing effort can predict the acceptance of user stories during sprint reviews}. Therefore, for this work, we will refer to \textit{external quality} as the \textit{Functional Suitability} as defined in IEC/ISO 25010 standard for software quality as they transpire in acceptance criteria attached to user stories~\cite{ISO25010}. 

The context of this study is a year-long software engineering project at the latest stages of undergrad studies. We observed 10 teams of 4 to 8 developers over 6 sprints (i.e. Scrum iterative cycles). We collected code coverage metrics calculated by testing frameworks (i.e. JUnit, Jest) together with manually calculated coverage of acceptance criteria attached to user stories (from Cucumber automated acceptance tests), as well as manual test scripts (in spreadsheets or wikis). We also analysed the teams' testing effort in terms of hours logged in Jira with special \textit{tags} passed in work-logs (e.g., \texttt{\#test}, \texttt{\#testmanual}, \texttt{\#fix}). In details, for each sprint:

\begin{enumerate}
\item we took snapshots of the code coverage of the produced software in terms of unit testing for each sprint deliverable;
\item we mapped automated and manual acceptance testing scripts to each acceptance criteria of the user stories that were planned for each delivery;
\item we evaluated the software products with a manual assessment of delivered user stories after each iteration of development, as a product owner would do during a Scrum sprint review;
\item we analysed the teams' testing effort in terms of hours logged as \texttt{\#test} and \texttt{\#testmanual}, in relation to the teams' effort to implement features or fix bugs, as retrieved from the teams' work-logs in Jira and Gitlab repositories.
\end{enumerate}

The remainder of the paper is organised as follows. We discuss the related work in Section~\ref{sec:rw}. We introduce the study setting and the method followed in Section~\ref{sec:method}. We present our results in Section~\ref{sec:results} and discuss these results in Section~\ref{sec:discussion} together with their implications to educators and practitioners as well as the limitations and threats to validity. We introduce the next steps and conclude in Section~\ref{sec:conclusion}.

\section{Related Work}
\label{sec:rw}

\subsection{Secondary Studies on Testing Practices}

Some secondary studies have investigated how some testing techniques may affect the external quality of software. 
Juristo \textit{et al.}~\cite{Juristo2004} then Vassalo \textit{et al.}~\cite{Gonzalez2014} classified testing techniques and evaluation metrics used, but did not address their effects on external quality in their literature reviews.
Bissi \textit{et al.} conducted the most recent systematic review on the effects of test-driven design on produced software, including on external quality~\cite{Bissi2016}. From that review, we discuss all relevant works to ours in the section below, i.e. \cite{Maximilien2003, Yenduri2006, Bhat2006, Slyngstad2008, Vu2009, Pancur2011}.
Abushama \textit{et al.} conducted a systematic literature review on the effects of test- and behaviour-driven design~\cite{Abushama2021}, from which one work is relevant to ours~\cite{Scandaroli2019}, also discussed below.
Van Heugten Breurkes \textit{et al.} conducted a systematic literature review on the overlap of automated unit and acceptance testing in industry context~\cite{vanHeugten2022}. The authors concluded that a test-first mindset can be beneficial without being able to demonstrate any further correlation.
Binamungu and Maro report on a mapping study about Behaviour-Driven Development (BDD) where they investigated the common themes and focus of prior studies where BDD has been applied~\cite{Binamungu2023}. We discuss hereafter the relevant papers to our focus, i.e. \cite{Dookhun2019, Rocha2021}.


\subsection{Test- and Behaviour-Driven Development}
% Need to talk aout BDD too
The literature on the effects of test-driven development (TDD) and, to a lower extent behaviour-driven development (BDD) is luxurious. In the following, we only consider case or longitudinal studies that have been conducted over an extended period of time (i.e. at least multiple weeks) in team-based environments.

\paragraph{In academia} 
Yenduri and Perkins reported a positive effect of TDD on the numbers of \textit{``faults''} in the code written by students over multiple months~\cite{Yenduri2006}. But no details are given on the complexity of the code written or how representative it is of the real world.
Vu \textit{et al.} performed a comparative case study in a capstone project with the industry~\cite{Vu2009}. However, the small sample size, the difference in the technology stack, and high mortality rate prevents to draw any insightful conclusions.
Huang and Holcombe run a project-based course over 12 weeks where students gather the requirements and develop a software for an external client~\cite{Huang2009}. The work is then evaluated following qualitative criteria only, but not extensively regarding its functional correctness.
Pančur and Ciglarič investigated the effects of TDD on the external quality of programming assignments with automated acceptance tests given to students in advance~\cite{Pancur2011}. In this work, we investigate the evolution of a larger scale project over time.
Lopes de Sousa \textit{et al.} introduced BDD into a Scrum-based software development of an academic tool where they observed benefits in terms of accurate translations between user stories and functional requirements~\cite{LopesdeSouza2017}. 
Baldassarre \textit{et al.} studied the ``retainment'' (\textit{aka} retention) of TDD by a student cohort over a six month period~\cite{Baldassarre2021}. Our objective is to observe the testing effort in general.
Santos \textit{et al.} conducted a meta analysis of twelve experiments conducted either in academia or industry to investigate, among others, the external quality of software produced under TDD practices~\cite{Santos2021}. Unlike other primary and secondary studies, TDD had a detrimental effect, however their baseline was not \textit{``pure waterfall''}, but a test-last approach in an iterative process made of short cycles. Our work complements these experiments by gathering more testing methods than TDD solely, i.e. acceptance and manual testing. 
Rocha \textit{et al.} report on their experience with students applying TDD and BDD in a software project course where they observed better grades and faster delivery~\cite{Roche2021}. However, the authors do not clearly specify whether the grades were directly linked to the external quality of the delivered software products.

\paragraph{Industry context} 
Bhat and Nagappan reported on multiple case studies where TDD was applied at Microsoft, resulting in a defect rate being halved compared to similar projects using a test-last approach~\cite{Bhat2006}.
Damm and Lundberg report on two projects where TDD was introduced for component-level testing and resulted in marginal decrease of defects being discovered at a later testing stage~\cite{Damm2006}.
Kobayashi \textit{et al.} introduced extreme programming practices into two software development projects and identified a positive effect on the code quality from interviews with developers~\cite{Kobayashi2006}.
Maximilien \textit{et al.}, then Sanchez \textit{et al.} reported on the shift to test-driven development (TDD) at IBM leading to a significant decrease in defect rates over multiple projects~\cite{Maximilien2003,Sanchez2007}.
Slyngstad \textit{et al.} discussed the shift to TDD after a few iterations of a development project with a significant decrease in defects rate~\cite{Slyngstad2008}.
Similarly to Santos \textit{et al.}~\cite{Santos2021}, Siniaalto \textit{et al.} identified a decreasing code quality when applying TDD in a comparative case study~\cite{Siniaalto2008}.
Bannerman and Martin observed that a \textit{``test-with-development''} approach decrease the code complexity on open source projects~\cite{Bannerman2011}.
Scandaroli \textit{et al.} report on the application of behaviour-driven design alongside TDD in two industry projects~\cite{Scandaroli2019}. They mention some benefits qualitatively (e.g., better alignment with business, higher acceptance of delivered features), but do not give evidence of such benefits in their experience report.
Dookhun\textit{et al.} reports an improvement in the external quality of software when BDD is used in conjunction to TDD, at the cost of a decrease in productivity and internal quality~\cite{Dookhun2019}.
Papis \textit{et al.} conducted an experiment where interns rotated between a no-unit-test, test-last or test-first methods to develop features in one-week iterations~\cite{Papis2022}. The authors identified a positive effect on the number of bugs introduced under test-first as well as for the code quality (assessed by pre-written acceptance tests).
Farooq \textit{et al.} conducted a systematic literature review of uses and applications of BDD where they concluded that BDD can address communication gaps between business stakeholders and developers and therefore improve the quality of software development processes as well the quality of the final product~\cite{Farooq2023}.

\paragraph{Our contribution} 
However, compared to all of the above, our work is the first to directly observe software development projects over an extended period of time where subjects must write both the code together with acceptance tests and manual tests. Furthermore, our contribution is the first to investigate the link between testing metrics (i.e. unit test coverage, implementation / testing effort, and coverage of acceptance criteria associated to user stories) and the external quality (i.e. functional correctness) of delivered products.


\subsection{Testing Effort And External Quality}

Some works have been proposed to analyse programming patterns and incentivize or give feedback to students on their programming behaviour, but not so much on their testing effort, as identified by Keuning \textit{et al.}'s literature review~\cite{Keuning2018}. From the list of tools, only a few are relevant to our work, that we discuss here. 

Edwards \textit{et al.} proposed Web-CAT, recently augmented with a gamification module, to encourage students to write more tests~\cite{Edwards2003,Buffardi2014,Edwards2020}. However, differences in external quality was marginal after the introduction of Web-CAT  and the gamification module still requires further validation. 
Helminen \textit{et al.} trace programming and testing behaviours of students in a web-based course~\cite{Helminen2013}. But the testing effort is observed from console-based interactions, not from structured automated testing.
Kazerouni \textit{et al.} defined a series of metrics to estimate the testing effort in students assignments and how these metrics can be used to predict the external quality of the software produced~\cite{Kazerouni2017,Kazerouni2019}. Similarly to many works discussed above, the authors observed a correlation between the external quality and an incremental testing method. However, the authors argued for a similar experiment to be conducted in a longer, larger project to validate their findings, which is our objective here.

\paragraph{Our contribution} We replicate the industry by limiting the \textit{``nudges''} we give to students to sprint reviews (i.e. passed stories), and feedback on testing effort in relation to the product's external quality. We are also interested in understanding the overall testing dynamics in a team-based environment, aspect that has not been analysed in previous works.

\subsection{Continuous Integration and Testing}
% TODO need more work to talk about testing, but still relevant
Usage by and perceptions of developers and stakeholders of continuous integration (CI) and more particularly, the role of automated testing in rapid or continuous software deployment (CD) has been researched extensively.
Ståhl and Bosch conducted a literature review on CI practices in the industry where they clustered related aspects of the usage of CI processes (e.g., scope, fault handling, build gfrequency)~\cite{Stahl2014}.
Gmeiner \textit{et al.} report on a 6 year long study of implementing a CI pipeline in an Austrian company with additional manual acceptance testing~\cite{Gmeiner2015}. 
Vassalo \textit{et al.} surveyed a financial industry to understand their CI/CD practices, including how they were testing their software~\cite{Vassalo2016}. 
Teixera \textit{et al.} conducted a systematic literature review on how DevOps can be characterised in terms of ``capabilities'' (e.g., testing, feedback loop) and ``areas'' (e.g., culture, process)~\cite{Teixeira2020}.
\paragraph{Our contribution} However, none of these works investigated the link between (unit and acceptance) testing methods or metrics, and the acceptance of delivered features by the user or product owner.


\section{Method}
\label{sec:method}

Our objective is to explore whether we can predict the success of a product delivery in a Scrum-based software development project from the testing behaviours and metrics of a team in terms of the accepted stories by the product owner. Specifically, our goal can be refined in the following research questions:

\begin{description}
\item[RQ1] How can we combine multiple test metrics to quantify the overall \textit{``testing effort''} in order to predict the functional suitability~\cite{ISO25010} of a software product in a Scrum-based project?
\item[RQ2] How does this \textit{``testing effort''} relate to the remedial effort a team of junior developers will put into fixing a software product during next Scrum sprint?
% \item[RQ3] How does the split between automated and manual tests evolves over the course of a Scrum-based project as the product grows?
\end{description}

To answer \textbf{RQ1}, we combine the following metrics into a \textit{testing effort} indicator and compare that metric to the number of successfully delivered stories after each sprint:

\begin{enumerate}
    \item code coverage from automated unit testing, i.e. functional correctness;
    \item coverage of acceptance criteria by automated acceptance testing (in \textit{Cucumber}), i.e. functional completeness;
    \item coverage of acceptance criteria by manual end-to-end system testing (retrieved from test records and spreadsheets), i.e. functional completeness;
    \item proportion of accepted user stories by the product owner, including their functional appropriateness;
    \item the time spent by developers writing automated tests or running manual tests.
\end{enumerate}

To answer \textbf{RQ2}, we compare the \textit{testing effort} indicator calculated above and compare it to:
\begin{itemize}
    \item the number of hours a team of junior developers spent testing their product, i.e. writing automated tests or running manual tests;
    \item the number of hours a team of junior developers spent fixing bugs.
\end{itemize}

% To answer \textbf{RQ3}, we observe the trends of testing coverage metrics computed in RQ1 over the course of a full year project course in software engineering with ten teams of junior developers.

\subsection{Study Design}

\subsubsection{Participants}

This study has been done on a whole year project course in the third year of Software Engineering degree at the University of Canterbury. At this point in the curriculum students already have a background in object-oriented software design in both Python and Java. The course has following prerequisites: introduction to object-oriented design and programming in Java, and database course. Students also need to take a software engineering course that covers Scrum, automated testing, continuous integration, and design patterns alongside the project course. At the start of the study, 80 students were fully enrolled in the course at the beginning of the year, with 70 completing the course from which 7 were identified as women, and 63 as men. We obtained appropriate approval from students to use their data for research purposes after anonymising them.

\subsubsection{Timeframe and Support}

The project ran for the full academic year (i.e. two semesters) with 6 sprints (i.e. iterations), each sprint being approximately 3 academic weeks long. All teams of 7 to 8 students worked on the same project at first, from a small template containing the initial technology stack, then diverged to create distinguishable products. Students were expected to log around 300 hours of work, as required per University regulations for typical project activities, e.g., Scrum events, implementation work, workshops and other contact hours. Some students have dropped the course after a few sprints as they realised that they will not fulfil the course requirements in terms of engagement. This has affected some teams more than others and created difference between teams in terms of number of students at the end of the year in each team.

Each scrum team was overlooked by a scrum master being a tutor, i.e. a student who passed the course previously. At the beginning of each sprint, teams discuss with the product owner (a course lecturer) their sprint commitment (number of stories they will take on). A course lecturer composes  product backlog and outlines acceptance criteria (AC) per each story. Additional teaching staff are overlooking the technology stack used by students, training and supervising the Scrum masters, and marking the software products (both documentation and code).

A specific workshop on acceptance testing strategies was offered at the beginning of the project (sprint 2). During this workshop students learnt how to write automated acceptance testing using \textit{Cucumber}. Both automated unit and manual acceptance testing were techniques taught and practised in previous courses that are prerequisites and co-requisites for this course. 

\subsubsection{Process}

The students were expected to follow the Scrum framework while working on the project course. Each sprint, students have gone through the following Scrum events:   
\begin{description}
    \item[Backlog grooming] go through a number of stories in the backlog, understand what work is required to complete them, update the acceptance criteria if needed;
    \item [Planning] teams agree on the stories they will work on in the current sprint with the product owner. Teams are then responsible to compose their sprint backlog by selecting which stories they pick up each sprint. Teams also have the opportunity to discuss their sprint commitment during a sprint to defer some stories, i.e. remove them from the sprint backlog, also called deferred stories.
    \item [Sprint] the actual time period when the scrum team works together to finish sprint backlog;
    \item [Stand-up:] status meeting (usually 15 min long) for teams, most of them supervised by Scrum masters or another teaching team member;
    \item [Sprint review] teams review each others' products against the acceptance criteria of each committed story (excluding the deferred stories); an additional product review is conducted by the teaching team;
    \item [Sprint retrospective] team reflects on the sprint that has just finished and decide on action items to improve their process.
\end{description}

\subsubsection{Delivery}

Each delivery is typically composed of a software product deployed on a virtual machine. The deployment follows a continuous integration (CI) pipeline triggered from a \textit{GitLab}\footnote{See \url{https://about.gitlab.com/}} repository hosted locally at the University. The continuous integration pipeline also contains dedicated automated testing stages, and is connected to a local \textit{SonarQube}\footnote{See \url{https://www.sonarsource.com/products/sonarqube/}} instance for students to keep track of their code quality metrics, including test coverage. Alongside the code, students have to keep a trace of their design decisions, manual testing logs, user interface mockups, user guide, and any additional documentation needed to run the project locally, all of these being part of the assessed material for each delivery (i.e. sprints).

Each delivery is followed by a comprehensive assessment by the teaching team including individual and team feedback about the functional suitability of the product, the quality of the code, the quality and amount of testing, the quality of the documentation and the ability for individuals and teams to follow the Scrum process.

% we don't need that many details 
%At the end of each sprint (set by date and time) students need to tag the commit, they would like to be considered as their deliverable for the sprint,  at their central repository (on UC's GitLab server) . Students are using continuous integration (CI) in this course so in our case, this averages that whenever someone pushes code to the team's central repository a tool called the GitLab Runner will trigger project build, execute tests and deploy the sprint product to Team's production environment. Each team is provided with a virtual machine (VM) hosted by UC on which to run the GitLab Runner. Every VM has production and testing environment. Students deploy to testing environment throughout the sprint to integrate their work gradually and test, while deployment to production happens only at the end of the sprint. GitLab runner follows the 'build rules' specified in .gitlab-ci.yaml file included at the root all official team project repos.

% this part is not relevant for this paper
%After each sprint teaching team gives students formal feedback about their individual and team performance for the sprint that just finished. Based on this feedback the students get the idea what grade they can expect by the end of the year if they continue to work as they do, but also what to improve on in the next sprint and beyond. 

%The product deployed to VM production environment is the one teaching team would assess for internal and external quality.


%- Should we talk about technologies used, spring framework, java, Junit, cucumber..?


%  In our case study students work on the year long project. Students (in teams) work in 2-3 weeks long life cycles (sprints). For the duration of the sprint, students are required to record their working session (should not be longer than 3 hours) in Jira. They are also required to tag their work (e.g.  #implementation, #test,#manualtest, #fix..). After each working session students also their code to central repository and record manual tests perform on GitLab wiki. By doing so, we have continusly update sources of data (Jira and GitLab) which we use to come up with the following matrics for assesing testing efforts:  

% - hours spent on testing during the sprint (automated testing, manual testing ) - Jira

% - test code coverage for both front-end and back-end part of the project, automated acceptance testing coverage and manual testing coverage  - GitLab

% The testing effort metrics are quantitative only as we do not examine the quality of executed tests.

% For coverage of acceptance criteria, a combination of the coverage of automated and manual tests is gathered, i.e. if there are 10 ACs (AC1-10), AC1-5 are covered by auto, AC4-7 covered by manual, then 70\% of ACs are covered.
% Our assumption is that this approach will give us an indicator on how many ACs have been attempted to be tested. We assume that some testing of AC is better than none and even though we do not know what the quality of testing is like the fact that students have spent time thinking about tests and writing them as part of their development process is going to bring the implementation features closer to the requirements. 
% As all of the students in the course had to do some courses as prerequisite we expect to roughly have similar level of testing knowledge and ability, so the quality of testing should be close to equal between teams.

\subsection{Data Sources}

We use multiple sources for data collection, including first-degree \textit{work diaries}~\cite{Lethbridge2005}, automatically calculated metrics, and teams test scripts. In this project course, students log their time spent on the project into a project management tool. We used \textit{Jira}\footnote{See \url{https://www.atlassian.com/software/jira}} where teams created their sprint backlogs and recorded their work logs, connected to \textit{GitLab} code commits. Work logs are composed of a short summary of the work done and the time spent on that task, i.e. ticket. Students are encouraged to log their time in a granular way, so a task will have multiple work logs. Additionally, students use prescribed tags to describe the work completed, close to Conventional Commits tags\footnote{See \url{https://www.conventionalcommits.org/}}, e.g., \texttt{\#implement} for implementation of features, \texttt{\#test} for writing automated tests, \texttt{\#testmanual} for writing or executing manual tests, and \texttt{\#fix} for bug fixing. One work-log can have multiple tags when appropriate, for example when students use test-driven development, they will typically tag a work log with both \texttt{\#test} and \texttt{\#implement} tags. In the following, we detail how we obtained the data described in Section~\ref{sec:method} we use to calculate our testing effort. One researcher carried the extraction, and a second researcher proofread the extraction and aggregation of data.

\subsubsection{Code coverage metrics} 
This is obtained by building sprint deliverable code. We access unit testing code coverage from \textit{JaCoCo}\footnote{See \url{https://www.jacoco.org/jacoco/}} reports uploaded to SonarQube when a deliverable is build by the CI pipeline. Code coverage is gathered from \textit{JUnit}\footnote{See \url{https://junit.org/} (Java)} and Jest\footnote{See \url{https://jestjs.io/} (JavaScript)} unit tests. For the purposes of this study we compiled the code coverage data for the delivered software products at the end of each sprint.

\subsubsection{Coverage of acceptance criteria from automated tests} 
Students are required to write automated acceptance tests on \textit{Gherkin}, i.e. \textit{Given-When-Then} syntax, as \textit{Cucumber} scenarios\footnote{See \url{https://cucumber.io/}}. Metrics about the number of scenarios are collected in the aforementioned \textit{JaCoCo} reports. However, there is no explicit relation between the number of \textit{Cucumber} scenarios and the coverage of an acceptance criteria, so we manually mapped scenarios to acceptance criteria. The acceptance criterion was considered fully covered if there was at least one acceptance test written for it.   

\subsubsection{Coverage of acceptance criteria from manual tests} 
To determine manual test coverage, we looked into the manual testing records teams made available on their GitLab wiki. Similarly to above, manual testing coverage was determined by mapping manual tests to acceptance criteria. The acceptance criterion was considered fully covered if there was at least one manual test written for it.

\subsubsection{Overall coverage of acceptance criteria} 
To determine overall acceptance test coverage, we have combined testing effort of acceptance testing using \textit{Cucumber} and manual testing by determining how many ACs were covered using either or both techniques combined. For example, if there are 10 ACs (AC1-10), AC1-5 are covered by auto, AC4-7 covered by manual, then 70\% of ACs are covered. This approach gives us a global indicator of the coverage of ACs for each product delivery, regardless of the technique, i.e. automated or manual.

\subsubsection{Assessment of functional suitability} 
\label{sec:func-suitability}
To determine how many stories passed or failed at the end of each sprint, markers from the teaching team reviewed the products based on the stories teams committed to at the beginning of the sprint. Markers were randomised between teams and sprints. During a sprint, teams had the ability to re-negotiate their initial sprint commitment with the product owner, and therefore, defer stories. Some of these deferred stories would eventually be picked up during a later sprints, often with a lower estimation, i.e. smaller number of story points, reflecting the estimated fixing effort to pass that story. The passing rate of stories is calculated from the final commitment, i.e. without counting the deferred stories as failed stories.

\subsubsection{Time effort}
\label{sec:time-effort} 
We extracted the number of hours teams have spent on various activities from their Jira work-logs. Each team member had to classify their work-logs with specific tags, similar to \textit{Conventional Commits}. We sum up hours logged for (1) implementation of features, i.e. \texttt{\#implement} work logs tags; (2) writing automated unit and acceptance tests, i.e. \texttt{\#test}; (3) writing or carrying manual (end-to-end) testing, i.e.\texttt{\#testmanual}; and (4) bug fixing, i.e. \texttt{\#fix}. Students could use other specific tags for other types of activities, such as \texttt{\#document} to record design decisions, or \texttt{\#chore} to work on their CI pipeline, but they are not relevant for this research. Also, students could tag their work-logs with more than one tag, where suitable, e.g., \texttt{\#implement} and \texttt{\#test} when applying a test-driven development method, or \texttt{\#implement} and \texttt{\#fix} when fixing and expanding on a failed story.

\subsection{Metrics}

From the data sources above, we compute the following metrics for testing, functional suitability, and time effort.

\subsubsection{Testing}

\paragraph{Front-End Unit Test (\textbf{FEUT}):} Unit test code coverage of front-end part (i.e. user interface) of the project, in percentage of covered lines of code. The data was obtained from \textit{SonarQube}.

\paragraph{Back-End Unit Test coverage (\textbf{BEUT}):} Unit test code coverage of back-end part (i.e. business logic layers) of the project, in percentage of lines of code. The data was obtained from \textit{SonarQube}.

\paragraph{Automated Acceptance Test coverage (\textbf{AAT}):} Automated test coverage of acceptance criteria (\textit{Cucumber} scenarios), in percentage of covered acceptance criteria. The data was aggregated from manual inspection of automated scenarios, i.e. \textit{Gherkin} features, mapped to acceptance criteria for all stories.

\paragraph{Manual Acceptance Test coverage (\textbf{MAT}):} Manual tests coverage of acceptance criteria, in percentage of covered acceptance criteria. The data was aggregated from manual inspection of manual test scripts mapped to acceptance criteria for all stories.

\paragraph{Overall Acceptance Test coverage (\textbf{OAT}):} Combined coverage of acceptance criteria from automated and manual acceptance tests, in percentage of acceptance criteria for all stories.


\subsubsection{Functional Suitability}

\paragraph{Passed Story Points (\textbf{PSP}):} Percentage of story points passed in the sprint review. Data is based on sprint marking information from manual assessment by the marker.

\paragraph{Deferred Story Points (\textbf{DSP}):} Percentage of story points deferred to a later sprint. Data is gathered from teams lowering their commitment during a sprint.

\paragraph{Re-committed Story Points (\textbf{RSP}):} Percentage of story points a team took on the current sprint which were either deferred stories from a previous sprint or failed stories that were re-committed to this sprint. That percentage is relative to the committed story points, excluding deferred stories, e.g., the team committed to 120 points, including 30 points belonging to re-committed stories, but deferred 20 points, then $RSP = ((120-20) \times 30) \div 100 = 30\%$. Points may differ from the sum of deferred and failed stories from previous sprint as not all failed/deferred stories were re-committed to, and/or their point estimates were changed from one sprint to the following.


\subsubsection{Time Effort}
\label{sec:metric-time-effort}

Sprints were not lasting for the same number of days and teams were of different sizes, so we use proportional time for time effort metrics.

\paragraph{Automated Testing Effort (\textbf{ATE}):} Relative number of hours spent writing test code for unit and acceptance tests compared to the total number of hours logged by the whole team. We do not distinguish time effort by type of automated testing as teams often go back and forth between unit and acceptance testing when validating features. This data is supplied by team members in their work-logs with \texttt{\#test} tags.

\paragraph{Manual Testing Effort (\textbf{MTE}):} Relative number of hours spent writing and running manual tests by the whole team. We do not distinguish between writing and running manual tests as this can be conducted in parallel, from our observations of students. This data is supplied by team members in their work-logs with \texttt{\#manual-test} tags.

\paragraph{Fixing Effort (\textbf{FE}):} Relative number of hours spent fixing feature (or test) code by the whole team. This usually happen when teams re-committed to failed stories and to a lower extent when teams discover issues during a sprint. This data is supplied by team members in their work-logs with \texttt{\#fix} tags.

\paragraph{Implementation Effort (\textbf{IE}):} Relative number of hours spent writing code for feature development by the whole team. As noted in Section~\ref{sec:time-effort}, these hours are sometimes combined with other tags, including \texttt{\#test} or \texttt{\#fix} tags. This data is supplied by team members in their work-logs with \texttt{\#implement} tags.


\section{Data Analysis} 

At the beginning of the project, teams start in sub-teams for on-boarding and engagement reasons and merge in their full teams from sprint 2, hence we collect data from the second sprint onward. We had 10 teams in total but two teams recorded incomplete data about their acceptance and manual testing, so we removed these two teams from the analysis as we were not able to calculate their testing metrics accurately. 
We first look at the evolution of the testing metrics and functional suitability for all teams, then, we report on students' work-logs about their time effort (see Table~\ref{tbl:team-metrics}).

\subsection{Evolution of Testing Metrics}

At the end of each sprint, we aggregated and calculated testing metrics, including average values over all sprints, for each of the eight teams over five sprints, as shown in Table~\ref{tbl:team-metrics}.

% 
%Product mapping:
%Team 1000 - A
%Team 100 - B
%Team 500 - C
%Team 400 - D
%Team 900 - E
%Team 800 - F
%Team 300 - G
%Team 200 - H

\begin{table*}[!ht]
    \centering
    \begin{tabular}{| l | l || r | r || r | r | r || r | r | r || r | r | r | r |}
    \hline
        \textbf{Team} & \textbf{Sprint} & \textbf{FEUT} & \textbf{BEUT} & \textbf{AAT} & \textbf{MAT} & \textbf{OAT} & \textbf{PSP} & \textbf{DSP} & \textbf{RSP} & \textbf{ATE} & \textbf{MTE} & \textbf{FE} & \textbf{IE} \\ \hline\hline
        \multirow{7}{*}{Team-A} & sprint 2 & 19.7 & 72.3 & 5.0 & 0.0 & 5.0 & 0.0 & 0.0 & 0.0 & 9.7 & 11.5 & 9.3 & 25.7 \\
         & sprint 3 & 36.3 & 70.3 & 2.9 & 0.0 & 2.9 & 8.7 & 0.0 & 23.1 & 20.1 & 2.1 & 5.5 & 23.4 \\
         & sprint 4 & 47.3 & 69.2 & 41.7 & 31.7 & 62.2 & 40.3 & 21.4 & 0.0 & 39.2 & 2.7 & 27.2 & 44.6 \\
         & sprint 5 & 54.5 & 76.2 & 59.3 & 40.0 & 69.7 & 81.0 & 0.0 & 11.9 & 30.8 & 0.2 & 21.5 & 37.3 \\
         & sprint 6 & 61.3 & 80.7 & 43.2 & 40.5 & 65.9 & 88.1 & 0.0 & 0.0 & 27.1 & 1.3 & 13.6 & 38.9 \\
         & \textit{average} & \textit{43.8} & \textit{73.7} & \textit{30.4} & \textit{22.4} & \textit{41.1} & \textit{43.6} & \textit{4.3} & \textit{7.0} & \textit{25.4} & \textit{3.6} & \textit{15.4} & \textit{34.0} \\ \hline\hline
         %& \textit{stdev} & \textit{16.4} & \textit{4.7} & \textit{25.1} & \textit{20.8} & \textit{34.1} & \textit{40.3} & \textit{9.6} & \textit{10.4} & \textit{11.2} & \textit{4.6} & \textit{8.9} & \textit{9.1} \\ \hline\hline
         
        \multirow{7}{*}{Team-B} & sprint 2 & 0.0 & 35.1 & 0.0 & 25.4 & 25.4 & 14.5 & 26.7 & 0.0 & 5.6 & 1.6 & 11.4 & 32.0 \\
         & sprint 3 & 1.9 & 36.4 & 4.6 & 36.2 & 37.7 & 0.0 & 45.1 & 29.9 & 14.2 & 1.2 & 9.8 & 18.3 \\
         & sprint 4 & 35.4 & 41.4 & 6.0 & 2.0 & 8.0 & 56.8 & 41.3 & 21.6 & 18.2 & 2.4 & 18.9 & 37.8 \\
         & sprint 5 & 48.9 & 43.8 & 0.0 & 96.7 & 96.7 & 80.0 & 0.0 & 31.7 & 25.3 & 0.1 & 15.0 & 33.2 \\
         & sprint 6 & 57.2 & 48.6 & 0.0 & 0.0 & 0.0 & 83.0 & 0.0 & 0.0 & 24.9 & 0.0 & 16.0 & 39.2 \\
         & \textit{average} & \textit{28.7} & \textit{41.1} & \textit{2.1} & \textit{32.0} & \textit{33.6} & \textit{46.9} & \textit{22.6} & \textit{16.6} & \textit{17.6} & \textit{1.1} & \textit{14.2} & \textit{32.1} \\ \hline\hline
         %& \textit{stdev} & \textit{26.5} & \textit{5.5} & \textit{2.9} & \textit{39.3} & \textit{38.2} & \textit{37.9} & \textit{21.7} & \textit{15.7} & \textit{8.2} & \textit{1.0} & \textit{3.6} & \textit{8.3} \\ \hline\hline
        
        \multirow{7}{*}{Team-C} & sprint 2 & 45.8 & 67.3 & 4.0 & 17.0 & 17.0 & 36.5 & 5.5 & 0.0 & 21.5 & 1.3 & 14.3 & 33.7 \\
         & sprint 3 & 61.4 & 82.5 & 45.3 & 16.2 & 52.6 & 71.7 & 0.0 & 3.8 & 29.7 & 1.1 & 13.0 & 29.2 \\
         & sprint 4 & 68.9 & 86.4 & 41.8 & 58.7 & 70.2 & 58.6 & 0.0 & 1.5 & 26.3 & 2.1 & 18.5 & 35.5 \\
         & sprint 5 & 72.9 & 84.2 & 33.1 & 59.5 & 65.0 & 58.1 & 25.9 & 27.9 & 26.3 & 2.9 & 18.4 & 35.5 \\
         & sprint 6 & 79.9 & 86.3 & 52.0 & 65.9 & 79.9 & 100.0 & 0.0 & 51.9 & 25.6 & 2.8 & 19.7 & 43.3 \\
         & \textit{average} & \textit{65.8} & \textit{81.3} & \textit{35.2} & \textit{43.5} & \textit{56.9} & \textit{65.0} & \textit{6.3} & \textit{17.0} & \textit{25.9} & \textit{2.0} & \textit{16.8} & \textit{35.4} \\ \hline\hline
         %& \textit{stdev} & \textit{13.0} & \textit{8.0} & \textit{18.7} & \textit{24.7} & \textit{24.4} & \textit{23.3} & \textit{11.2} & \textit{22.6} & \textit{2.9} & \textit{0.9} & \textit{2.9} & \textit{5.1} \\ \hline\hline
         
        \multirow{7}{*}{Team-D} & sprint 2 & 10.9 & 67.3 & 3.1 & 84.0 & 82.1 & 85.2 & 16.9 & 3.7 & 20.1 & 17.2 & 30.6 & 44.9 \\
         & sprint 3 & 21.7 & 68.2 & 38.3 & 76.7 & 86.7 & 38.2 & 0.0 & 8.8 & 15.5 & 15.5 & 19.7 & 30.0 \\
         & sprint 4 & 31.9 & 70.6 & 47.7 & 63.6 & 73.0 & 35.1 & 8.1 & 3.5 & 21.9 & 3.9 & 10.3 & 35.9 \\
         & sprint 5 & 38.6 & 69.7 & 33.6 & 77.5 & 83.3 & 100.0 & 0.0 & 14.0 & 19.4 & 4.3 & 12.3 & 35.2 \\
         & sprint 6 & 56.8 & 73.4 & 0.0 & 89.6 & 89.6 & 95.6 & 0.0 & 0.0 & 24.7 & 4.5 & 12.8 & 29.9 \\
         & \textit{average} & \textit{32.0} & \textit{69.8} & \textit{24.5} & \textit{78.3} & \textit{82.9} & \textit{70.8} & \textit{5.0} & \textit{6.0} & \textit{20.3} & \textit{9.1} & \textit{17.1} & \textit{35.2} \\ \hline\hline
         %& \textit{stdev} & \textit{17.4} & \textit{2.4} & \textit{21.6} & \textit{9.7} & \textit{6.3} & \textit{31.7} & \textit{7.5} & \textit{5.4} & \textit{3.4} & \textit{6.7} & \textit{8.3} & \textit{6.1} \\ \hline\hline
         
        \multirow{7}{*}{Team-E} & sprint 2 & 12.7 & 42.2 & 0.0 & 0.0 & 0.0 & 32.3 & 0.0 & 0.0 & 21.3 & 1.1 & 20.3 & 32.8 \\
         & sprint 3 & 47.9 & 45.9 & 0.0 & 0.0 & 0.0 & 7.5 & 43.7 & 20.0 & 22.8 & 3.1 & 24.2 & 55.4 \\
         & sprint 4 & 58.1 & 46.5 & 2.3 & 88.9 & 88.9 & 85.9 & 28.3 & 43.7 & 25.7 & 3.1 & 23.6 & 41.7 \\
         & sprint 5 & 62.1 & 80.5 & 2.3 & 70.0 & 70.0 & 54.5 & 0.0 & 45.5 & 26.6 & 8.0 & 21.4 & 49.2 \\
         & sprint 6 & 55.2 & 79.2 & 3.7 & 71.4 & 73.3 & 75.8 & 0.0 & 0.0 & 14.6 & 8.9 & 23.9 & 42.1 \\
         & \textit{average} & \textit{47.2} & \textit{58.9} & \textit{1.7} & \textit{46.1} & \textit{46.4} & \textit{51.2} & \textit{14.4} & \textit{21.8} & \textit{22.2} & \textit{4.8} & \textit{22.7} & \textit{44.2} \\ \hline\hline
         %& \textit{stdev} & \textit{20.0} & \textit{19.2} & \textit{1.6} & \textit{42.7} & \textit{43.0} & \textit{32.0} & \textit{20.4} & \textit{22.3} & \textit{4.8} & \textit{3.4} & \textit{1.8} & \textit{8.5} \\ \hline\hline
         
        \multirow{7}{*}{Team-F} & sprint 2 & 32.7 & 69.0 & 26.0 & 0.0 & 26.0 & 27.8 & 0.0 & 0.0 & 21.7 & 2.9 & 24.5 & 49.0 \\
         & sprint 3 & 36.7 & 74.3 & 25.4 & 31.6 & 47.1 & 7.2 & 0.0 & 1.0 & 20.0 & 0.0 & 23.4 & 47.6 \\
         & sprint 4 & 42.4 & 68.2 & 21.6 & 22.3 & 37.9 & 72.0 & 16.3 & 2.4 & 18.0 & 1.9 & 32.0 & 45.3 \\
         & sprint 5 & 55.9 & 73.7 & 19.8 & 88.9 & 91.3 & 40.6 & 39.6 & 0.0 & 22.2 & 6.9 & 28.6 & 47.5 \\
         & sprint 6 & 51.7 & 74.9 & 1.6 & 31.7 & 37.0 & 100.0 & 0.0 & 45.8 & 15.0 & 0.8 & 26.8 & 44.0 \\
         & \textit{average} & \textit{43.9} & \textit{72.0} & \textit{18.9} & \textit{34.9} & \textit{47.9} & \textit{49.5} & \textit{11.2} & \textit{9.9} & \textit{19.4} & \textit{2.5} & \textit{27.1} & \textit{46.7} \\ \hline\hline
         %& \textit{stdev} & \textit{9.8} & \textit{3.2} & \textit{10.0} & \textit{32.8} & \textit{25.4} & \textit{36.7} & \textit{17.4} & \textit{20.1} & \textit{2.9} & \textit{2.7} & \textit{3.4} & \textit{2.0} \\ \hline\hline
         
        \multirow{7}{*}{Team-G} & sprint 2 & 57.2 & 32.3 & 23.3 & 5.6 & 28.9 & 88.4 & 10.4 & 0.0 & 18.0 & 0.0 & 15.4 & 38.6 \\
         & sprint 3 & 60.8 & 31.4 & 18.1 & 8.3 & 26.4 & 100.0 & 0.0 & 0.0 & 11.9 & 0.0 & 8.1 & 29.7 \\
         & sprint 4 & 65.7 & 38.6 & 0.0 & 0.0 & 0.0 & 21.7 & 36.1 & 21.7 & 12.9 & 0.0 & 11.8 & 22.2 \\
         & sprint 5 & 69.5 & 39.8 & 46.7 & 0.0 & 46.7 & 38.2 & 0.0 & 0.0 & 15.6 & 0.0 & 5.2 & 20.5 \\
         & sprint 6 & 74.5 & 40.5 & 14.8 & 4.4 & 19.3 & 81.1 & 0.0 & 8.1 & 18.0 & 0.0 & 10.3 & 36.0 \\
         & \textit{average} & \textit{65.5} & \textit{36.5} & \textit{20.6} & \textit{3.7} & \textit{24.2} & \textit{65.9} & \textit{9.3} & \textit{6.0} & \textit{15.3} & \textit{0.0} & \textit{10.2} & \textit{29.4} \\ \hline\hline
         %& \textit{stdev} & \textit{6.9} & \textit{4.3} & \textit{17.0} & \textit{3.6} & \textit{16.9} & \textit{34.0} & \textit{15.6} & \textit{9.5} & \textit{2.8} & \textit{0.0} & \textit{3.8} & \textit{8.1} \\ \hline\hline
         
        \multirow{7}{*}{Team-H} & sprint 2 & 11.7 & 51.5 & 4.8 & 0.0 & 53.6 & 75.9 & 0.0 & 0.0 & 13.8 & 3.1 & 17.8 & 42.6 \\
         & sprint 3 & 30.5 & 58.7 & 60.0 & 77.8 & 92.1 & 64.4 & 25.3 & 0.0 & 25.9 & 1.0 & 10.5 & 28.0 \\
         & sprint 4 & 30.2 & 47.0 & 58.7 & 56.1 & 79.0 & 76.4 & 0.0 & 11.5 & 27.9 & 3.4 & 18.6 & 46.1 \\
         & sprint 5 & 32.2 & 72.8 & 62.5 & 77.8 & 86.7 & 83.7 & 0.0 & 0.0 & 24.8 & 0.8 & 20.7 & 33.9 \\
         & sprint 6 & 33.9 & 74.6 & 50.8 & 98.2 & 98.2 & 87.7 & 24.4 & 0.0 & 26.8 & 3.1 & 21.6 & 37.9 \\
         & \textit{average} & \textit{27.7} & \textit{60.9} & \textit{47.4} & \textit{62.0} & \textit{81.9} & \textit{77.6} & \textit{9.9} & \textit{2.3} & \textit{23.8} & \textit{2.3} & \textit{17.9} & \textit{37.7} \\\hline
         %& \textit{stdev} & \textit{9.1} & \textit{12.4} & \textit{24.2} & \textit{37.7} & \textit{17.4} & \textit{8.9} & \textit{13.6} & \textit{5.1} & \textit{5.7} & \textit{1.3} & \textit{4.4} & \textit{7.1}
        
    \end{tabular}
    \caption{Test metrics (FE UT, BE UT, AAT, MAT, OAT), metrics for stories (SP, DP, RP), and time efforts (ATE, MTE, FE, IE).}
    \label{tbl:team-metrics}
\end{table*}


\subsubsection{Unit testing (FEUT, BEUT)}
Teams A, C, D and F maintained a relatively high back-end testing (BEUT) coverage in average, close to or above 70\% for all sprints, with C also putting significant effort in their front-end testing (FEUT). Team B had a low test coverage overall, slowly reaching 57.2\% (FEUT) and 48.6\% (BEUT) by the end of the project. Team E and Team G had low coverage overall with reversed focus, Team E invested more in their back-end, where Team G focused more on their front-end. Team H slowly improved their FEUT over the course, still keeping a low coverage on that side of the code, but significantly improved their back-end testing for the final two sprints, with a back-end coverage above 70\%. Team G was the only team with a higher FEUT than BEUT in average.

\subsubsection{Automated acceptance testing (AAT)}
AAT coverage values remained low for all teams. Two teams (B and E) never engaged much with automated acceptance testing overall. Three teams (A, C and H) did a better job with some sprints showing AAT coverage above 50\%, especially Team H for all but its first sprint. The remaining three teams (D, F and G) had a similar behavioural pattern with some effort put at first or sporadically, but disengaged with automated acceptance testing later on.

\subsubsection{Manual acceptance testing (MAT)}
\label{sec:mat}
Team C and H had a generally increasing manual testing coverage, with sustained effort across all sprints. Teams D and H especially increased their coverage during the last sprint with 90\% and 98\% coverage respectively, Team D has recorded lots of manual testing at first, then dropped to 39\% in sprint 4, and increasing sharply after. Teams A and E started to put effort in manual testing from sprint 4, but Team A kept a low coverage, where Team E stayed above 70\% MAT. Teams B and F had a push in manual coverage in sprint 5, but relatively low coverage elsewhere. 

\subsubsection{Overall acceptance testing (OAT)}
For all teams, there appear to be an overlap between automated acceptance and manual testing, sometimes significant, where teams likely tested the same acceptance criteria with both techniques. Except from Team G, we observe relatively close values between their overall coverage (OAT) and either their automated (AAT) or their manual acceptance (MAT) coverage. Teams B and F had erratic manual and overall testing behaviours where they significantly increased their acceptance test coverage in sprint 5 only. Team E never engaged with automated acceptance testing, but pushed their manual testing coverage for the last three sprints, hence a high OAT coverage for those sprints.

\subsubsection{Additional observations about testing effort}
Team D completely switched to manual acceptance testing in sprint 5, but recorded no acceptance testing for the final sprint with marginally improved unit testing coverage. Team B did not record any manual testing for sprint 6. Team G recorded very low coverage of (manual) acceptance testing overall, as well as low unit testing of their back-end, shifting most of their coverage effort on the front-end of their product. Team E increased their back-end and manual testing from sprint 4, but did not engage with automated acceptance testing.


\subsection{Evolution of Functional Suitability}

At the end of each sprint, a marker reviewed the delivered product and calculated the percentage of points passed, deferred and re-committed for each team, as shown in Table~\ref{tbl:team-metrics}.

\subsubsection{Passed Story Points (PSP)}
Teams A and B had a slow start but steadily improved over sprints with a high percentage of stories delivered in their last sprint (88\% and 83\% resp.). Interestingly, Team A, and to a lower extent Team B, started to pass significantly more stories when they started to show evidence of better test coverage metrics (mostly AAT and OAT for Team A, FEUT for Team B), as visible in Figure~\ref{fig:team-a}. However no similar trend is visible for any other teams. Teams C, D, E, F and G were irregular in their delivered stories, Team D being the second most successful team, with high BEUT and OAT. Teams C and F started low, but passed all their stories in the last sprint, with Team C showing the highest automated testing coverage values for that sprint across all teams, where F had very low acceptance testing. Team E delivered well in Sprints 4 and 6 only. Team D and G followed a similar pattern where they both started well, then dropped significantly for two sprints (Sprints 3 and 4 for Team D, and 4 and 5 for Team G), but finished well in the last sprint, with 96\% and 81\% passed story points respectively without observable relation to their testing metrics. Team H maintained a relatively high percentage of passed story points over all sprints, with their worst delivery at 64\% in sprint 3 and an average of 77.6\% points delivered, as visible in Figure~\ref{fig:team-h}. However, they had the lowest FEUT coverage, fifth BEUT coverage, but the highest AAT (47.6\%) and OAT (72.2\%) coverage in average.

\begin{figure}[h!]
\includegraphics[width=.49\textwidth]{images/Team-1000.png}
\caption{Testing coverage metrics and accepted stories for Team A}
\label{fig:team-a}
\end{figure}

% TODO make that picture better, especially for legend, mayber using R?
% \begin{figure}[h!]
% \includegraphics[width=.49\textwidth]{images/Team-500.png}
% \caption{Testing coverage metrics and accepted stories for Team C}
% \label{fig:team-c}
% \end{figure}

\begin{figure}[h!]
\includegraphics[width=.49\textwidth]{images/Team-200.png}
\caption{Testing coverage metrics and accepted stories for Team H}
\label{fig:team-h}
\end{figure}

\subsubsection{Deferred Story Points (DSP)}
All teams had two deferrals, except for Team B with 3 deferrals (in sprints 2, 3 and 4) and Team A with only one in sprint 4. Teams C, F and G had a similar deferral record with two deferrals, a smaller one followed by a larger one later on. Teams D and E had also two deferrals, but their first one was larger than their second one. Team H was the only team deferring stories in the last sprint. Team B deferred an average of 22.6\%, deferring the largest amount of story points in these sprints, where Team A deferred the lowest in average (4.2\%). There is no visible trend or relation between the DSP and the test metrics from visual observation.

\subsubsection{Re-committed Story Points (RSP)}
Re-committed stories typically accounted for a lower percentage than the combination of failed and deferred points from the previous sprint for all teams. Furthermore, some teams did not explicitly recommitted to failed stories, but ``absorbed'' the fixes into other stories, i.e. they did not recommit to the whole story, but either dropped it or combined it with another related story. 

Team E is the only team where we observe a visible relation between failed or deferred stories in one sprint, and an increase of re-committed story points in the next sprint, hence the highest value for recommitted story points. Team C explicitly recommitted to a big part of their stories in the last two sprints, where Team F did the same for their last sprint only, both teams' last commitment being made of more than 46\% of re-committed stories. Apart from Team E where an increase in re-committed story points partially matched an increase in testing, no other team showed noticeable trends.


\subsection{Evolution of Time Effort}
\label{sec:time-effort}

Table~\ref{tbl:team-metrics} summarises the relative hours spent by teams on the tasks of interest compared to the total time worked during that sprint, according to students' work-logs (4 last columns). As mentioned in Section~\ref{sec:time-effort}, some work-logs may contain more than one tag, so we cannot sum up hours with different tags for a sprint since some recorded hours would be counted twice. However, we calculated average effort values to support our discussion in comparison to passed stories (PSP) and testing coverage values (BEUT, FEUT, AAT, MAT).

% do we even need this now that we know the data is not to be trusted
\subsubsection{Automated Testing Effort (ATE)}

Team C put a consistent effort in automated testing, with an average of 25.9\% being the highest effort across all teams, with consistently high coverage metrics (except in sprint 2). However, they had the fourth average PSP rate across all teams, at 65\%, where, on the other hand, Team G had the lowest effort at 15.3\% in average, for a slightly higher average PSP rate at 65.9\%.

Teams A and B show a similar trend in their automated testing effort (ATE) across all sprints, with a low effort at first, increasing for a few sprints, then decreasing slightly. They exhibit a higher proportion of passing story points (PSP) one sprint after putting more effort in automated testing. However, while Team B spent a slightly lower proportion of their time writing automated tests than Team A, their PSP rate was similar despite significantly higher test coverage for Team A for all of FEUT, BEUT and AAT. Team G had the lowest automated testing effort overall with Team B, below 18\%, but Team G had higher coverage values for FEUT and AAT, and the third highest value of PSP, where Team A has the second highest effort in ATE and the lowest PSP rate on average.

Teams D, E, and F had similar average ATE with comparable coverage values, except for Team E's AAT. However no observable relationship to their respective PSP can be seen, e.g., Team E had similar ATE in sprint 4 and 5 where their BEUT coverage jumped in sprint 5 with other coverage values being close to sprint 4 ones, Team F had a drop in sprint 6 with 15\%, but delivered all stories.


\subsubsection{Manual Testing Effort (MTE)}

Teams A and D recorded a high MTE for sprint 2, with Team D also logging more than 15\% of their time on manual testing in sprint 3. Despite consistent high MAT coverage, changes in Team D's effort does not match changes in their manual coverage. Furthermore, Team A's MAT does not match their effort either, with 0 MAT coverage in sprint 2 despite 11.5\% MTE. The other teams also have logged very little effort in manual testing, with Team G logging 0 hours during the whole project despite some very limited MAT coverage. Therefore, apart from Team D to some extent, we believe all other teams did not log their manual testing effort properly, so this effort data is more than likely unreliable.


\subsubsection{Fixing Effort (FE)}
\label{sec:fe}
Teams have been logging between 10.2\% (Team G) and 27.1\% (Team F) of FE in average over all sprints. Sprint 4 was generally seeing the highest proportion of FE for most teams across all sprints, even if some teams, i.e. Teams C, and G had relatively high PSP in sprint 3. We have anecdotally observed a similar trend over the past years in the course due to accumulating technical debt and teams spending time to fix UI inconsistencies.

Where no observable relationship to passed stories (PSP) can be seen, it is worth noting that, from our observations, \texttt{\#fix} tags were also used for fixing technical debt by some teams, hence the numbers cannot be fully trusted.

\subsubsection{Implementation Effort (IE)}

Implementation efforts ranged from 18.3\% (Team B in Sprint 3) to 55.4\% (Team E in Sprint 3). Team G logged the lowest average implementation effort (29.4\%) where Team F logged the highest effort (46.7\%) on top of being very consistently high, above 44\% for all sprints. Five teams spent approximately a third of their time implementing features (Teams A, B, C, D, H) in average where Teams E and F logged more than 44\% IE in average. From manual observations, implementation efforts do not seem to influence or be influenced by other types of efforts, i.e. an increase in IE does not generally decrease other types of effort.


%Escape special TeX symbols (%, &, _, #, $)
%Compress whitespace    Smart output formatting

\subsection{Linear Regression via Mixed Model}
\label{sec:lmer}

To help us analyse the effect of different testing metrics on functional suitability and remedial effort in subsequent sprint, we have undertaken statistical modelling. For this purpose we have used \textit{R}\footnote{Sources available next to raw data at \url{TOBEADDED}}, a language and environment for statistical computing. We have used Linear Mixed-Effect model (LMER), an extension of linear regression for grouped data, as we have repeated observations of clusters of data, i.e. testing and time metrics per team, where teams can be considered as the random effect. Sections~\ref{sec:it-psp} to~\ref{sec:tte-psp} investigate RQ1 where Sections~\ref{sec:test-next} to~\ref{sec:psp-fe} relate to RQ2.


\subsubsection{Effect of Individual Testing Metrics on Passed Story Points (PSP}
\label{sec:it-psp}

We examine fixed affects in terms FEUT, BEUT, AAT, and MAT on passed stories, i.e. PSP, while taking into account a random effects in terms of the observed Teams. Table~\ref{tbl:team-metrics-stats} summarises the results, where we consider $Pr\leq0.05$ significant (identified by $**$) and fitted the model using the following expression in R.

\begin{empheq}{align*}
    m \leftarrow lmer(PSP \sim FEUT+BEUT+AAT+MAT+(1|Team))
\end{empheq}

\begin{table}[htb]
\begin{tabular}{|l|l|l|l|l|l|l|}
\hline
            & Estimate & St.Error & t value & Pr(>|t|)     \\ \hline
(Intercept) & 0.3159   & 0.1723   & 1.834   & 0.07522      \\
FEUT        & 0.6323   & 0.2188   & 2.890   & 0.00657  **  \\
BEUT        & -0.3307  & 0.2950   & -1.121  & 0.26984      \\
AAT         & 0.1731   & 0.2179   & 0.6311  & 0.794        \\
MAT         & 0.3895   & 0.1401   & 2.779   & 0.00871 **   \\\hline
\end{tabular}
 \caption{Fixed effect of testing metrics on passed stories using Linear Mixed-Effect model.}
    \label{tbl:team-metrics-stats}
\end{table}

From Table~\ref{tbl:team-metrics-stats}, front-end unit testing (FEUT) and manual acceptance testing (MAT) have statistically significant effect on passed story points (PSP) if other involved independent variables stay unchanged.
For every 1\% increase in FEUT or MAT, we can expect 0.63\% and 0.38\% increase in PSP respectively. Interesting, we believe that
because the BEUT metric remained high for most teams while their PSP rate vary from sprints to sprints has resulted in a negative relationship between these two metrics, i.e. the more teams put efforts in back-end testing, the lower they deliver, which seems counter-intuitive.

\subsubsection{Effect of Average Test Coverage (AVGTC) on Passed Story Points (PSP)}
\label{sec:avgtc-psp}

The previous model investigated the effect individual testing metrics have on passed story points. We now investigate whether the average of FEUT, BEUT and OAT testing, denoted AVGTC, is a better predictor of passed story points than each coverage alone. To this end, we used the following R calculation, with the results summarised in Table~\ref{tbl:team-TTC_stats}:

\begin{empheq}{align*}
    m \leftarrow lmer(PSP \sim AVGTC+(1|Team))
\end{empheq}

\begin{table}[htb]
\begin{tabular}{|l|l|l|l|l|l|l|}
\hline
            & Estimate & St.Error & t value & Pr(>|t|)     \\ \hline
(Intercept) & 0.06858  & 0.14390  & 0.477   & 0.637449     \\
AVGTC       & 0.98650  & 0.25997  & 3.795   & 0.000628 *** \\\hline
\end{tabular}
 \caption{Fixed effect of average testing coverage on passed story points.}
    \label{tbl:team-TTC_stats}
\end{table}

The results from Table~\ref{tbl:team-TTC_stats} show that the average test coverage has a statistically significant effect on PSP. Moreover, the combined testing coverage has a greater effect on PSP compared to individual techniques. Based on the estimation value in Table~\ref{tbl:team-TTC_stats}, each percent increase of AVGTC would create a 0.98\% increase of PSP. In other words, in order to reliably increase the probability to pass a story, a team would need to invest in all types of testing, i.e. cover a story at the unit, acceptance, and manual (or end-to-end) level, all together.


\subsubsection{Effect of Testing (ATE \& MTE), Fixing (FE) and Implementation Efforts (IE) on Passed Story Points (PSP)} 
\label{sec:effort-psp}

We discussed in Section~\ref{sec:time-effort} that, from manual observations, time logs are potentially unreliable. However, we want to inspect whether the time spent on various activities, i.e. automated testing, manual acceptance testing, fixing and implementation, has any statistically significant effect on passed story points (PSP). We applied the following R function, with its results shown in Table~\ref{tbl:team-effort-stats}.

\begin{empheq}{align*}
    m \leftarrow lmer(PSP \sim ATE+MTE+FE+IE+(1|Team))
\end{empheq}

\begin{table}[htb]
\begin{tabular}{|l|l|l|l|l|l|l|}
\hline
            & Estimate & St.Error & t value & Pr(>|t|)  \\ \hline
(Intercept) & 0.1182   & 0.2662   & 0.444   & 0.660     \\
ATE         & 1.0573   & 0.8975   & 1.178   & 0.250     \\
MTE         & -0.8777  & 1.4831   & -0.592  & 0.561     \\
FE          & 0.4276   & 1.2849   & 0.333   & 0.741     \\
IE          & 0.5365   & 0.9515   & 0.564   & 0.577     \\\hline
\end{tabular}
 \caption{Fixed effect of testing efforts on passed story points.}
    \label{tbl:team-effort-stats}
\end{table}

From the results in Table~\ref{tbl:team-effort-stats}, none of the recorded efforts have a statistically significant effect on past story points, i.e. $Pr\geq0.05$ for all combinations.

\subsubsection{Effect of Total Testing Effort (TTE) on Passed Story Points (PSP)} 
\label{sec:tte-psp}

We aggregate the total testing effort (TTE) as the sum of automated and manual test efforts (i.e. ATE + MTE) and investigate its effect on passed story points, with the following R formula, generating the results in Table~\ref{tbl:team-TTC_stats}. 

\begin{empheq}{align*}
    m \leftarrow lmer(PSP \sim TTE+(1|Team))
\end{empheq}

\begin{table}[htb]
\begin{tabular}{|l|l|l|l|l|l|l|}
\hline
            & Estimate & St.Error & t value & Pr(>|t|)  \\ \hline
(Intercept) & 0.3535   & 0.1779   & 1.987   & 0.0542    \\
TTE         & 0.9611   & 0.7005   & 1.372   & 0.1781    \\\hline
\end{tabular}
 \caption{Fixed effect of total testing effort on passed story points.}
    \label{tbl:team-TTC_stats}
\end{table}

Similar to Section~\ref{sec:effort-psp}, we do not see any statistically significant correlation between total testing effort and past story points, i.e. the time students spend at writing automated tests does not predict the number of story points they will deliver.

\subsubsection{Estimation of Testing Coverage metrics (FEUT, BEUT, AAT, MAT, AVGTC) on Fixing Effort (FE) in the Following Sprint} 
\label{sec:test-next}

Our second objective, i.e. RQ2, investigates whether we can estimate the remedial effort in a subsequent sprint from testing coverage metrics in the previous sprint. To this end, we examine the relation between the fixing effort of the next sprint (denoted $fix.next$ below) and the testing coverage metrics, i.e. BEUT, FEUT, AAT, MAT, AVGTC in the current sprint with the following R formula:

\begin{empheq}{align*}
    m \leftarrow lmer(Fix.next \sim FEUT+BEUT+AAT+MAT+AVGTC(1|Team))
\end{empheq}

\begin{table}[htb]
\begin{tabular}{|l|l|l|l|l|l|l|}
\hline
             & Estimate  & Std. Error & t value & Pr(>|t|)  \\\hline
(Intercept)  &  0.12414  & 0.05980    &  2.076  & 0.0516    \\
FEUT         &  0.06811  & 0.12304    &  0.554  & 0.5846    \\
BEUT         &  0.14009  & 0.13364    &  1.048  & 0.3043    \\
AAT          &  0.03481  & 0.06552    &  0.531  & 0.6004    \\
MAT          &  0.07238  & 0.07941    &  0.911  & 0.3718    \\
AVGTC        & -0.18923  & 0.27196    & -0.696  & 0.4940    \\\hline
\end{tabular}
 \caption{Fixed effect of testing metrics on fixing effort in the following sprint.}
    \label{tbl:team-metrics_to_Fix.next_stats}
\end{table}

The results of the LMER model are represented in the Table \label{tbl:team-metrics_to_Fix.next_stats}. None of the testing metrics have a statistically significant effect on the fixing effort in the following sprint, following our intuition from the analysis in Section~\ref{sec:fe}. However, it remains unclear whether this is due to poor logging and tagging from students.


\subsubsection{Estimation of Total Testing Effort (TTE) on Fixing Effort (FE) in the Following Sprint} 
\label{sec:tte-fenext}

For the purpose of checking if testing in one sprint impacts the time spent on remedial work in the following sprint, we check whether the total testing effort (TTE, calculated as ATE + MTE) influences the fixing effort in the following sprint. We executed the following R formula, with its result shown in Table~\ref{tbl:team-TTE_stats}.

\begin{empheq}{align*}
    m \leftarrow lmer(Fix.next \sim TTE+(1|Team)) % teams have been sampled repeatedly \\
\end{empheq}

\begin{table}[htb]
\begin{tabular}{|l|l|l|l|l|l|l|}
\hline
            & Estimate & St.Error & t value & Pr(>|t|)  \\ \hline
(Intercept) & 0.10093  & 0.03877  & 2.603   & 0.0147 *  \\
TTE         & 0.30828  & 0.13904  & 2.217   & 0.0346 *  \\\hline
\end{tabular}
 \caption{Fixed effect of total testing effort on fixing effort in the following sprint using Linear Mixed-Effect model}
    \label{tbl:team-TTE_stats}
\end{table}

From Table~\ref{tbl:team-TTE_stats} we see that testing in one sprint predicts a slight increase in fixing effort during the next sprint. To further inspect the relationship between testing and fixing effort, we also investigate the same trend per individual sprint, as visible in Figure~\ref{fig:TTE_on_Fix_per_sprint}, where the coloured lines represents the trend for all teams per sprint.

% m <- lmer(Fix.next ~ TTE*Sprint+(1|Team), data=d) # teams have been sampled repeatedly
% dft <- expand.grid(TTE = seq(0,.5,length.out=101),Sprint=sort(unique(d$Sprint))[1:4])

% dft$y <- predict(m,dft,re.form=~0)

% ggplot()+
%   geom_point(data=d,aes(x=TTE,y=Fix.next,
%                         col=Sprint))+
%   geom_line(data=dft,aes(x=TTE,y=y,col=Sprint))

\begin{figure}[htb]
\centering
\includegraphics[width=.49\textwidth]{images/TTE_Fix_next_per_sprint.png}
\caption{Effect TTE has on Fix.next per sprint}
\label{fig:TTE_on_Fix_per_sprint}
\end{figure}

As we can see from Figure ~\ref {fig:TTE_on_Fix_per_sprint}, for all but Sprint 3, the fixing effort in the next sprint (denoted ``Fix.next'') increases as the total testing effort (TTE) increases. This further support our initial intuition regarding incorrect and unreliable effort logging from students. Another plausible explanation would be that tests must be rewritten or adapted the next sprint, so an increase in automated tests increases the test codebase that needs to be maintained later on. We will expand on these findings in Section~\ref{sec:limitiations} where we go over the limitations of our study.


\subsubsection{Estimation of fixing effort (FE) in the following sprint based on past story points (PSP) in the current sprint}
\label{sec:psp-fe}

In order to refine our intuition around wrong effort logging and tagging by students, we investigate whether the amount of remedial work needed in the following sprint is influenced by the number of story points a team passed the previous sprint. In other words, intuitively, we would expect a higher proportion of time spent implementing fixes after a failed delivery (i.e. low functional suitability), where a successful delivery would mean less time spent on fixes the next sprint. To this end, we run the following R formula, with its results shown in Table~\ref{tbl:team-PSP-on-Fix.next-stats}.

\begin{empheq}{align*}
    m \leftarrow lmer(Fix.next \sim PSP+(1|Team))
\end{empheq}

\begin{table}[htb]
\begin{tabular}{|l|l|l|l|l|l|l|}
\hline
            & Estimate & St.Error & t value & Pr(>|t|)      \\ \hline
(Intercept) & 0.17056  & 0.02624  & 6.500   & 9.09e-06 ***  \\
PSP         & 0.01043  & 0.03139  & 0.332   & 0.742         \\\hline
\end{tabular}
 \caption{Fixed effect of passed story points on next sprint's fixing effort.}
    \label{tbl:team-PSP-on-Fix.next-stats}
\end{table}

There is no statistically significant correlation between passed stories and fixing effort in the following sprint. We believe that this lack of correlation further support our observation regarding inaccurate work logging.

% \subsection{Correlation of Testing Metrics and Functional Suitability}

% Based on the statistical modelling we can see that direct correlation between percentage of overall test coverage and percentage of passed stories per sprint (functional suitability). 
% This trend is particularly obvious for Teams C and Team H . Figures~\ref{fig:team-c} and \ref{fig:team-h} visually show the improvement in testing coverage together with the assessment of the functional suitability.

% Team C started with reasonable level of backend unit test coverage but very low acceptance testing, hence functional suitability, (product quality) is only ~40\% of story points. The product quality has increased to over 70\% and has continued to increase in sprint 6 reaching the total of 100\% success rate. This seems to be related to the increase of automated acceptance testing and manual testing in sprint 4 \& 5. During sprint 6 most teams focus on testing and/or fixing (see Table 2) as this is their last sprint and product was to be prepared for the final presentation to the wider audience (the department and industry). Therefore, it is not surprise that most of the teams have improved the product quality in the last sprint.

% Team H had reasonable level of backend and acceptance testing right through the project and consequently the functional suitability was stable throughout the year (on ~80\% on average).

% The exception to this trend can be observed in Team F. The team has had continuously high back-end unit testing but low front-end unit testing and acceptance testing throughout the year. Their functional suitability has been very unstable. The fluctuation in product quality was going in the opposite direction to the acceptance testing trend (e.g. when manual testing was at its pick in sprint 5, the functional suitability dropped significantly). This required inspection of additional influencing factors. 

% Team F seems to have performed better when the sprint was including a break (term or semester break). When a sprint was worked on during term time only, they seem to have struggled to produce a high product quality (sprint 3 \& 5). This could be related to the fact that this was a team of high performing individuals who worked hard on other courses during a term and therefore they focused on the project course more over the break, as there was a bit of flexibility to do so. Therefore the code quality and testing effort seem to have improved during these sprints (sprint 4 \& 6).

% Also, in sprint 5 manual acceptance testing significantly improved (2.5 x increase from previous sprint), but the functional suitability didn't follow. This was curious so we looked further.
% %and we looked at the manual testing coverage on AC level. Looking at the manual tests produced we noticed that they tried to increase the coverage by having only 1 manual test for each AC. Even though we assume that AC is covered if there is at least on manual test written for it, this often is not enough, and having such light coverage does not guarantee functional suitability for every AC.

% We noticed that in sprint 5 Team F had a very optimistic sprint estimate/commitment which lead to huge deferral ( 40\% of story points, see DSP, Table ~\ref {tbl:team-metrics}). The team had to spend some time on these stories but the effort didn't pay off as they decided to defer. This effort doesn't contribute to current sprint outcome but does increase success rate of the next sprint as students have already put some thoughts into those stories (and potentially wrote some code for it). Based on the difference between passed story and passed story points percentage, we can conclude that they have passed simpler stories and stories that failed in the previous sprint but that they have failed and deferred more complex ones, new/unfamiliar stories.
% In sprint 6, they reached very high level of functional suitability even though the testing effort appeared to have dropped (see Figure 7, sprint 6). In this sprint they have 46\% of redeemed story points suggesting that half of the backlog was made out of deferred and failed stories from previous sprint. These are the stories that they worked on before and were easier to get right due to their previously acquired knowledge. At this stage the testing seems to have been mostly on the development level, therefore not always logged.




% - Should I be looking at the following data where we are observing lack of product quality while testing was high :
%     - Team dynamics
%     - sicknesses
%     - other course work and lack of planning of their time
%     - over committing and lack of planning
%     - not enough experience with automated acceptance testing (high testing \% in that case doesn't necessary average the high product quality)
%     - ?

% Some of the possible reasons why teams did well in-spite of the low testing stats:
% - gained experience in technology they were using over time, so less problems introduced 
% - working on fixes not complex new implementation
% - change of marker? 

% - Is it worth adding a bit of maths to this by seeing what is the standard deviation for correlation between high testing and high quality, or is the sample of data too small to look into this.

%  Team-G presented another example of inconsistent testing and quality. This team has invested in front-end testing mostly (unit testing for Jest) while back-end and automated acceptance testing was on the average to low level. Manual testing was almost non-existable and automated acceptance testing was done but inconsistently. This suggests that testing strategy focused on front-end testing only does not result in desirable product quality. This conclusion is supported by comparing this team to Team-H were front-end testing was low but the overall product quality was high, due to high level of coverage in back-end, automated acceptance testing and manual testing. 

% Team E has had somewhat similar pattern to Team F. They have deferred 44\%  of stories in sprint 3 and have then worked on these stories in sprint 4. This previously acquired knowledge would have given them a significant advantage when working on these stories. They also significantly increased their manual testing coverage in sprint 4. Those two factors seem to have had a combined effect on their success rate in sprint 4 (~80\%).

% In sprint 5 they have deferred 28\% of story points. By looking at the passing story points rate (lower than a story passing rate) they seem to have focused on easier stories and deferred more complex ones. This kept they product quality on reasonably high level of ~80\%. By looking at the graph for Team-E, sprint 5, manual acceptance testing coverage seems lower then in sprint 4, even though they have spent more hours manual testing (~25h in sprint 5, compared to ~12h in sprint 4). This is a bit miss-leading as they seem to have written (and executed) more tests per story in sprint 5. They have had 53 manual tests over 4 stories compared to 50 manual tests over 9 stories in sprint 4. So, the manual testing effort was still very high (even though not quite reflected through the coverage)  which seemed to has keep the product quality at high level. We can observe the similar behaviour in sprint 6.

% Team D was the team that if we were to look at the overall testing coverage and story passing rate it would appear that testing didn't directly made any difference to their success rate (especially in sprint 3 and 4). For example, in sprint 4, the team had low product quality (35\% of story points passed), while overall acceptance testing was on a reasonable level (71\%). When inspecting the acceptance testing on individual story level (more granular data not available in the paper) we could see that they had very low number of acceptance tests per AC (often only 1) , but as we (for practical reasons) assume that AC is covered if there is at least one acceptance test (automated or manual ) implemented, we have considered these stories fully tested. For some ACs one test per AC does not cover all potential scenarios covered in an AC, and quite a few stories failed as a result. 
% % do we want to mention that having one manual test per AC might be a problem, as it might affect the validity of our initial assumtion

% In sprint 5, even though overall acceptance testing dropped to 50\%, they have passed all stories. Again, this required a closer inspection of the sprint commitment and acceptance testing records. In this sprint, 6/10 stories worked on, were failed stories from previous sprint. So only small fixes have been required. The team knew exactly what needs fixing based on the feedback they got from the teaching team. These stories didn't have high level of acceptance testing but as only minor fixes were required, there was less of a chance that something would go wrong. Other 4 (new) stories have been fully acceptance tested and therefore passed the review. So, this team success rate still very much depended on the level of testing they have done.
% Team A has failed large portion of their stories in the first 3 sprints and have put many hours towards fixing their issues in sprint 4. They also improved in all aspects of testing from sprint 4 onwards. This is the sprint where we have seen the first significant improvement in the product quality. The fact that they deferred 1/5 of their commitment in this sprint also helped with success rate (if they haven't deferred, they would have most likely failed them). In sprint 5 \& 6 they further increased FEUT, BEUT AAT (in sprint 5 only) and MAT. We could see significant improvement in PSP in these two sprints too.

% Team B has not been very consistent with the way they have been recording their acceptance testing (manual testing mostly). Often it was hard to determine a match between a test and an AC.  This has resulted in somewhat inconclusive picture. In sprint 2 \& 3 they had very low unit test coverage (below 40\%) , same goes for acceptance test coverage. It is therefore not a surprise to see that their PSP was very low too (14.5\% and 0\% respectively )  They have had a high deferral rate in sprints 2 \& 3 \& 4 and consequently high redeemed story points rate in 3 \& 4 \& 5, which suggests that they had trouble estimating and planning sprint commitment in those sprints.  In sprint 4 they have managed to pass over 50\% of story points even though their manual testing and automated acceptance testing dropped significantly. Which could be due to the high redeemed story points rate (worked on the stories they have failed in previous sprints). They have also continuously increased their front-end and have had a close to full coverage of manual acceptance testing in sprint 5 resulting. This improvement in FEUT and MAT followed by the improvement in PSP goes in line with previously found correlation between front-end unit testing and functional suitability. 

% In sprint 6, team didn't have any manual or automated acceptance testing, while both front-end and back-end unit testing has increased only by a little (~10\% increase) but have still managed to reach a highest level of PSP (83\%). They worked on 4 new, good size stories (8-13 points), so didn't have any redeemed story points in their commitment, but yet managed to do well. This confirms that increase in FEUT is making a significant impact to product quality (as fund in statistical analysis)

%Team-A has spent many hours on testing but not much on manual testing while they still have some manual tetsing coverage. I wonder if they logged it all under test tag. For example in sprint 5 they have had 31 tests but have spent only 0.6h on manual testing. Is this even possible to do?

% Do we need this now???
% The pattern of teams work distribution over time is another important aspect of team work and their impact on overall product quality (functional suitability). To get this overview we have look at summary of time teams spent on specific tasks per sprint. We have collected the worklog data and calculated  the percentage of total logged time spent on fixes, testing (automated and manual) and implementation. We have looked for correlation between the portion of time spent on testing and the actual test coverage as well as if there is consequential increase in hours spent on fixes followed by a poor deliverable.  
% As discussed in Data Sources section, students have used project management tool \textit{Jira}\footnote{See \url{https://www.atlassian.com/software/jira}} to classify and log time spent on the project. The tags we are mostly interested here are those related to implementation, testing (automated and manual) and fixes (see Table 1).   

% % do we need this paragraph we have covered this laready elsewhere

% It is worth noting that, often students would use more than one tag to record the time spent in a session. For example, when they work on a new feature but also write unit tests in the process, they would log their total time spent using \#implementation and \#test tag. The total time logged would have been added to both tag summaries (e.g. a 3h session with tags \#implementation and \#test would have increased both tags total for that sprint for 3h hours).  Therefore this metric should be used to determine a trend of work distribution for teams over the time rather than an absolute (accurate) value of total time spent on the project. 

% Team F: 
% By looking at the hours they spent on various activities (see Table 2) we can notice that they spent many hours fixing issues from sprint 3 (the sprint with lowest product quality) in sprint 4. This resulted in second highest number of hours spend on fixes any team had for the duration of the year - 154.4h ( see Table 2). Similar thing happened in sprint 6 for Team F, number of hours spent on fixing increased after an unsuccessful sprint 5 (just over 40\% of passed stories).
% Team F also seem to have had a problem with planning and estimation even later in the year. They were the team of strong, overconfident individuals which put the high expectations on themselves.   More specifically in sprint 3 they passed only 7\% of story point (see SP column in Table 1). In sprint 4 they seem to have spent a lot of time fixing the sprint 3  issues (see Table 2, fix tag for sprint 4)  
% The product quality for sprint 4 appears to be much higher than in sprint 3. Testing and fixing effort has increased (Table 2) .

% In sprint 6 team has reduced an overall testing effort, while fixes and new features implementation hours have increased. This is another example of drop in product quality sprint (sprint 5) followed by a sprint with increased fixing effort.  As this was the last sprint spent a lot of time fixing the product and preparing for the final delivery. This seem to have helped the team reach high product quality.
% Overall, this team did better when they have spent more time fixing issues (not necessary testing). The way the fixing has been done here could be associated with white box testing, when a developer examines the written code and subsequently test locally made changes (bug fixes). It is obvious that they would have benefited from more thorough overall acceptance testing during the sprint.

% Team E spent many hours fixing issues from sprint 3 which, as we have seen with Team-F, often boosts the passing rate (small code changes followed by manual testing). Overall manual testing effort has increased significantly in sprint 4 which improved overall acceptance testing coverage and subsequently the product quality (to 86\% passing story points in sprint 4). 

% Team A -This team seem to have logged all their testing hours under the test tag, as we can see the effort put towards testing from sprint 4 onwards has significantly increased. They seem to have logged most of their manual testing under this tag too, as effort logged under manual testing tag does not matched the number of test written and run. For example, in sprint 5 they have had 31 manual tests in total but have only logged 0.6h under manual testing.
% %


%Discuss handling of mortality
%Discuss the fact that markers are changing from sprint to sprint so there is some subjectivity when marking.
% Must talk about MAT being acceptance testing-driven

%\subsubsection{Validity procedure}

%cite ~\cite{Runeson2012}

\section{Discussion}
\label{sec:discussion}

From collected data and performed analysis we can see that if a team of third year students working on a year long project has had continuously had high level of overall
acceptance testing (manual testing and automated acceptance testing combined) and mid to high level of front-end testing,
they are most likely going to reach a high product quality. We have observed this behaviour with Team H and C.
Any combination of low or inconsistent acceptance testing but higher back-end unit testing (Teams F, E, A)  or higher acceptance testing but very low front-end unit testing (Team D) or high front-end testing only ( Team G) or low testing overall (Team B) would not produce a functionally stable, high quality product. This finding implies that only regular and incremental testing (both unit and acceptance testing) needs to be perform from the early stages of the development to unsure a satisfactory product quality. 

Statistical modelling has showed us that some types of testing have greater impact on product quality in the year long university project. We have seen that both front-end unit testing and manual testing play a crucial part in the project success. This suggests that testing techniques that are close to user experience seem to be more helpful in achieving high level of story acceptance rate in the early stages of project development.

We know that BDD (behavior driven development) has shown some positive impact on external product quality ~\cite{Farooq2023} in industry. We were expecting to see similar impacts of this development technique in the university project. Based on data we collected and statistical analysis performed we cannot confirm this to be the case. 
This could be for the following reasons:
\begin{enumerate}
\item This testing technique is new to the students. They only learn the basics of how to use it at the start of the course. They seem to struggle to apply it to a more complex scenarios later in the year and therefore use it either sparingly or inadequately (simple scenarios only).
\item It has already been noted that there is a decrease in productivity when using BDD and ATDD due to the lack of experience of the programmers who had little or no experience for this technique ~\cite{Dookhun2019}. Extensive training might have been required for this technique to use adequately. 
\item The size of the project by the end of the year is still relatively small, using manual testing alone as acceptance testing technique is feasible. 
\end{enumerate}

% Team G  testing effort data looks stange. They have had a big drop in quality but do not have many hours spent on fixes.

As we have seen in Linear regression for mixed models analysis we cannot draw any significant correlation between worklog data and past story points or effect of testing on fixing effort in the next sprint.\\
There could be various reasons for lack of correlation between logged effort and success rate of the project.
The most likely one is related to the fact that students individual grades in the course were directly affected by the number of hours logged against various activities.\\
This has in return somewhat influenced the distribution of hours they logged per sprint. For example, they were advised that every development activity needs to be accompanied with testing activity (ideally both unit and acceptance testing).
It seems that some students have abused the system in order to appear they have done enough of implementation and/or testing per every session. This can be concluding based on the fact that automated testing is reasonably stable through out year for all teams, while we have seen reasonable fluctuation in testing coverage.
It also appears that manual testing effort was not logged accurately and that some of this effort has been logged using \#test tag ( an automation testing tag). We have concluded this as some teams have had high manual testing coverage in one sprint but had very low manual testing effort logged (e.g. Team B, sprint 5).\\
Same goes for fixing effort, where teams have used the \#fix tag not only for fixing issues found in previous sprints but also to fix issues found in code review, chores (development environment tasks, VM set up), UI clean ups and similar (e.g.Team D, sprint 2 ).


\subsection{Summary of Findings}
\textit{What testing strategy should junior developers follow?}
Based on limited data we have, we can conclude that high level of unit testing (both back-end and front-end) is beneficial but on its own cannot assure the product quality. Acceptance testing plays an important role in ensuring that customers' requirements are met. In our study case we have looked at both manual acceptance testing and automated acceptance testing. We have seen that in a year long project manual testing seems to have had a superior impact on product quality compared to automated acceptance testing. This could be different in a team of senior developers but for junior developers systematic manual testing seems to be more beneficial acceptance testing technique. 

\textit{Can lack of testing in one sprint be compensated for in the later sprints}
Teams that have had a low level of testing in one sprint found it hard to recover from it in the later sprints. While small improvements are possible (e.g. Team A \& B) it is very hard to reach a high product quality in the following sprint in testing is not incorporated into development practice from a very early on.
This is in line with ~\cite{Kazerouni2017}, where was suggested that earlier and regular testing (both unit and acceptance testing) leads to higher product quality.  

\textit {Can a team of junior developer master the skill of BDD and ATDD in a year long project course} Based on our case study, BDD and ATDD are not easily acquire development techniques. It appears that students being all equally inexperienced in using these techniques at the start of the project course, do not have enough time and opportunity to learn how to implement more complex scenarios. This is more likely to be different in industry where teams often have a mixture of senior and junior developers and higher level of knowledge sharing and mentoring exists.
%Check whether we arrive to the same conclusions as ~\cite{Kazerouni2017}.

\subsection{Limitations}
\label{sec:limitations}

\textit{Testing metrics are quantitative} : Acceptance test coverage records for both manual and automated acceptance testing are both determined by manually mapping a written test to an acceptance criteria.  The acceptance criteria was considered fully covered if there was at least one manual test (or automated acceptance test/scenario written for it.  There is a possibility that one automated or manual acceptance test doesn't fully cover the acceptance criteria.

\textit{The quality of written tests hasn't been taken into account}: The quality of acceptance tests are not closely examined. There is a possibility that some of the tests do not in fact test the right thing or that scenarios is not complete (some parts of the tests are missing). 

\textit {Work-log can have more than one tags}: we can't determine how much time is spent on each activity with accuracy. For example, 3h sessions logged with tags \#implement, \#test and \#testmanual, suggests that a student has spent 3h working on all those activities, but how much they spent on each of those activities individually, it is not possible to tell. This could be the reason why proportion of effort logged against testing didn't fluctuate much per sprint/team.
\textit {Work-log recording might depend on/be influenced by hours expectation set by the teaching team}: When marking students teaching team expects to see an even spread of implementation and testing hours in the work-log (among other things). It seems that (some) students have tried to game the system by logging hours worked on the project based on our expectations rather than on their actual work. This has potentially created a level of noise in the logged effort data. This is less likely to be the problem with testing metrics (testing coverage) as these purely depend on actual tests written.  

\textit {Inconsistent logging of manual testing effort}: Manual testing effort depended on team's decision on how these will be recorded.
Some teams have high amount of hours logged under test, but almost none under manual testing. Team B for example, seem to have a good manual testing coverage in sprint 5 , but only 0.1\% of total time was logged against this tag. We assume that they have used \#test tag for both unit testing and manual testing effort logging. Same teams have very low or none manual testing coverage in some sprints but have achieved the high level of PSP (e.g. Team G, sprint 3 and Team F, sprint 6). It is very unlikely that they managed to achieve this by unit testing only, so we will regard this lack of manual records (and acceptance testing in general) as noise rather than a true reflection of the testing done. 

\textit {Fixing effort included wide range of activities}: On some instances (as for team B, sprint 6) team has spent a reasonable amount of time fixing issues while no redeemed story points were claimed. This suggests that \#fix tag was not always used appropriately and might have been used to log other type of work (UI redesign or code refactoring for example).


\subsection{Threats to Validity}

% refer to \cite{Zampetti2020} about design of course (implications to educators)
\textit{Internal Validity}
\begin{enumerate}
\item Instrumentation : There was an assumption that AC is covered if it has at least one manual test or automated acceptance test was written for it. If a team manually tested an AC without recording manual test we would consider it uncovered. 
\item Instrumentation ? : The information on how much time was spent on each activity depends solely on students' work-log. The number of hours students log directly impacts students grades, it is possible that students didn't log accurately to meet the expectations.
\item Time recording: One work-log session can cover more than one activity, therefore logging for example, 3h for the session while using \#test, \#Implementation and \#fix tag would increase the total time for each of these categories for 3h. 
\item Confounding : The end of sprint product marking has been done by group of academics and tutors. There was a random rotation of markers, to ensure that a product was not marked by the same marker every sprint. This has potentially cause a slight variation in PSP values per team per sprint.
\item Confounding : Some sprints were going over the study breaks. This has had a slight impact (for some positive for some negative) on sprint outcome. Some teams chose to work over the break which improved their delivery, but most have planned to work over the break but have in fact been distracted with other courses so have removed themselves for development work for a significant period of time, making it harder to get back to it.
\item Attrition : Some students have dropped out of the course half way through the year. This could have made an impact on some of the coverage results ( e.g. having less members would have change the team focus from quality of delivery to features only). It would also mean that results obtained from one sprint to another might differ due to having less people available to do the work.



\end{enumerate}
\textit{External Validity}
\begin{enumerate}
\item Hawthorne effect (or Observer bias?) : Students are thought (in previous courses and in the project course under study) that every development activity needs to be accompanied with testing. They are also aware that we expect them to spend at least 1/3 of their development time testing. This could have influenced the amount of testing they do (and log).
\item Population: Students are put into teams manually. The attention is to have a mix of race, gender and ability (we look at the data we have from previous courses). By forming the teams in this way we are setting a similar level of diversity within each team and therefore avoid selection bias.

\end{enumerate}
\textit{Construct Validity}
\begin{enumerate}
% Construct validity is essentially the degree to which our scales, metrics and instruments actually measure the properties they are supposed to measure
\item Is test code coverage the right unit testing measure? A metric that is commonly used to measure the adequacy of testing is code coverage. We have therefore used this metrics to determine thoroughness of a project test suit. This metrics however does not take into account the quality of test suite. We had to assume that 3rd year students are proficient enough in writing unit tests by this stage of their studies.
\item Acceptance testing code coverage calculation. We have assumed that an AC is acceptance tested if it has at least one automated acceptance test or manual test written for it. We haven't taken into account the quality and thoroughness of these tests (do they cover all aspects of an AC).
\item Product quality metrics. We have used past story points (PSP) as a measure of product quality/functional suitability. This measure does not take into account usability, ease of use, speed and similar other non-functional requirements.
\end{enumerate}




% \subsubsection{Mining Contributions on Gitlab} % Do we need this?
% %TODO, does this apply to our case study, as we do not look at individual contribution , and only check end of sprint deliverables, so do we mind squash commits, rebase....?
% cite \cite{Bird2009} on pitfalls of git mining (i.e. we don't let them to rebase, no squash commits, only simple merge with history preservation, we merge aliases to same author, similar main + dev + feature / task branches)

% rely on work-logs from students, including logs with multiple tags, e.g., one 3h session with both implement and test tags

% Issue with sprints over breaks 

% Survivorship bias

% Incentives and their impact

% Mortality affecting teams more than others, check with Alyssa's Team 

\section{Conclusion and Future work}
This paper presented the results of case study aimed at assessing which combination of testing techniques contributes best to the product quality in a year long university project. It also looked at correlation between testing in one development iteration and effort spend on fixing issues in the following iteration (sprint). The case study involved 8 teams made out of 5-8 students over period of 6 sprints. 

The results show that there is statistically significant correlation between past story points (referred to as product quality) and amount of manual acceptance and front-end unit testing done in one sprint. Back-end unit testing and automated acceptance testing coverage have not shown any significant impact on product quality. Back-end unit testing was high for most teams and therefore appeared not to have an impact on product quality in isolation.
Automated acceptance testing was not used to the full potential. We concluded that students were not very proficient in using this testing technique and have struggled to use it with more complex scenarios.
We have also not observed any significant correlations between testing done in one sprint and fixing effort in the following sprint. There are number of reasons why this was not the case, as discussed in Limitations.

For the future work we suggest the following:
\begin{enumerate}
\item Improve how we teach BDD and ATDD. In this year students didn't use automated acceptance testing to its full potential. They seemed to have struggle with harder scenarios. In order to make this more approachable to students we might need to offer more than one workshop on this topic. One at the start of the year and one at the mid year. We also could introduce a knowledge sharing session for students to exchange their experiences and ways to overcome common issues.
\item Improve logging guidance to create a more specific instructions for students on how to log their work in order to achieve more accurate logging.  
\item Having a firmer guidance on product marking to minimise the impact of marker's bias on PSP.
\item Manual testing recording needs to have a consistent /prescribed structure to make the coverage calculation more accurate
\item In this research we only looked at code coverage (unit tests) and acceptance test coverage (manual testing and automated acceptance testing). In order to know how well tests cover a feature we need to look at the quality of tests too.
\end {enumerate}


\label{sec:conclusion}

==> tables.tex <==
% ACM compliant full table

\begin{table*}[!ht]
    \caption{Test metrics (FEUT, BEUT, AAT, MAT, OAT), metrics for stories (SP, DP, RP), and time efforts (ATE, MTE, FE, IE).}
    \label{tbl:team-metrics}
    \begin{tabular*}{\textwidth}{| l | l || r | r || r | r | r || r | r | r || r | r | r | r |}
    \hline
        \textbf{Team} & \textbf{S\#} & \textbf{FEUT} & \textbf{BEUT} & \textbf{AAT} & \textbf{MAT} & \textbf{OAT} & \textbf{PSP} & \textbf{DSP} & \textbf{RSP} & \textbf{ATE} & \textbf{MTE} & \textbf{FE} & \textbf{IE} \\ \hline\hline
        \multirow{6}{*}{A} &  2 & 19.7 & 72.3 & 5.0 & 0.0 & 5.0 & 0.0 & 0.0 & 0.0 & 9.7 & 11.5 & 9.3 & 25.7 \\
         &  3 & 36.3 & 70.3 & 2.9 & 0.0 & 2.9 & 8.7 & 0.0 & 23.1 & 20.1 & 2.1 & 5.5 & 23.4 \\
         &  4 & 47.3 & 69.2 & 41.7 & 31.7 & 62.2 & 40.3 & 21.4 & 0.0 & 39.2 & 2.7 & 27.2 & 44.6 \\
         &  5 & 54.5 & 76.2 & 59.3 & 40.0 & 69.7 & 81.0 & 0.0 & 11.9 & 30.8 & 0.2 & 21.5 & 37.3 \\
         &  6 & 61.3 & 80.7 & 43.2 & 40.5 & 65.9 & 88.1 & 0.0 & 0.0 & 27.1 & 1.3 & 13.6 & 38.9 \\
         & \textit{avg} & \textit{43.8} & \textit{73.7} & \textit{30.4} & \textit{22.4} & \textit{41.1} & \textit{43.6} & \textit{4.3} & \textit{7.0} & \textit{25.4} & \textit{3.6} & \textit{15.4} & \textit{34.0} \\ \hline\hline
         %& \textit{stdev} & \textit{16.4} & \textit{4.7} & \textit{25.1} & \textit{20.8} & \textit{34.1} & \textit{40.3} & \textit{9.6} & \textit{10.4} & \textit{11.2} & \textit{4.6} & \textit{8.9} & \textit{9.1} \\ \hline\hline
         
        \multirow{6}{*}{B} &  2 & 0.0 & 35.1 & 0.0 & 25.4 & 25.4 & 14.5 & 26.7 & 0.0 & 5.6 & 1.6 & 11.4 & 32.0 \\
         &  3 & 1.9 & 36.4 & 4.6 & 36.2 & 37.7 & 0.0 & 45.1 & 29.9 & 14.2 & 1.2 & 9.8 & 18.3 \\
         &  4 & 35.4 & 41.4 & 6.0 & 2.0 & 8.0 & 56.8 & 41.3 & 21.6 & 18.2 & 2.4 & 18.9 & 37.8 \\
         &  5 & 48.9 & 43.8 & 0.0 & 96.7 & 96.7 & 80.0 & 0.0 & 31.7 & 25.3 & 0.1 & 15.0 & 33.2 \\
         &  6 & 57.2 & 48.6 & 0.0 & 0.0 & 0.0 & 83.0 & 0.0 & 0.0 & 24.9 & 0.0 & 16.0 & 39.2 \\
         & \textit{avg} & \textit{28.7} & \textit{41.1} & \textit{2.1} & \textit{32.0} & \textit{33.6} & \textit{46.9} & \textit{22.6} & \textit{16.6} & \textit{17.6} & \textit{1.1} & \textit{14.2} & \textit{32.1} \\ \hline\hline
         %& \textit{stdev} & \textit{26.5} & \textit{5.5} & \textit{2.9} & \textit{39.3} & \textit{38.2} & \textit{37.9} & \textit{21.7} & \textit{15.7} & \textit{8.2} & \textit{1.0} & \textit{3.6} & \textit{8.3} \\ \hline\hline
        
        \multirow{6}{*}{C} &  2 & 45.8 & 67.3 & 4.0 & 17.0 & 17.0 & 36.5 & 5.5 & 0.0 & 21.5 & 1.3 & 14.3 & 33.7 \\
         &  3 & 61.4 & 82.5 & 45.3 & 16.2 & 52.6 & 71.7 & 0.0 & 3.8 & 29.7 & 1.1 & 13.0 & 29.2 \\
         &  4 & 68.9 & 86.4 & 41.8 & 58.7 & 70.2 & 58.6 & 0.0 & 1.5 & 26.3 & 2.1 & 18.5 & 35.5 \\
         &  5 & 72.9 & 84.2 & 33.1 & 59.5 & 65.0 & 58.1 & 25.9 & 27.9 & 26.3 & 2.9 & 18.4 & 35.5 \\
         &  6 & 79.9 & 86.3 & 52.0 & 65.9 & 79.9 & 100.0 & 0.0 & 51.9 & 25.6 & 2.8 & 19.7 & 43.3 \\
         & \textit{avg} & \textit{65.8} & \textit{81.3} & \textit{35.2} & \textit{43.5} & \textit{56.9} & \textit{65.0} & \textit{6.3} & \textit{17.0} & \textit{25.9} & \textit{2.0} & \textit{16.8} & \textit{35.4} \\ \hline\hline
         %& \textit{stdev} & \textit{13.0} & \textit{8.0} & \textit{18.7} & \textit{24.7} & \textit{24.4} & \textit{23.3} & \textit{11.2} & \textit{22.6} & \textit{2.9} & \textit{0.9} & \textit{2.9} & \textit{5.1} \\ \hline\hline
         
        \multirow{6}{*}{D} &  2 & 10.9 & 67.3 & 3.1 & 84.0 & 82.1 & 85.2 & 16.9 & 3.7 & 20.1 & 17.2 & 30.6 & 44.9 \\
         &  3 & 21.7 & 68.2 & 38.3 & 76.7 & 86.7 & 38.2 & 0.0 & 8.8 & 15.5 & 15.5 & 19.7 & 30.0 \\
         &  4 & 31.9 & 70.6 & 47.7 & 63.6 & 73.0 & 35.1 & 8.1 & 3.5 & 21.9 & 3.9 & 10.3 & 35.9 \\
         &  5 & 38.6 & 69.7 & 33.6 & 77.5 & 83.3 & 100.0 & 0.0 & 14.0 & 19.4 & 4.3 & 12.3 & 35.2 \\
         &  6 & 56.8 & 73.4 & 0.0 & 89.6 & 89.6 & 95.6 & 0.0 & 0.0 & 24.7 & 4.5 & 12.8 & 29.9 \\
         & \textit{avg} & \textit{32.0} & \textit{69.8} & \textit{24.5} & \textit{78.3} & \textit{82.9} & \textit{70.8} & \textit{5.0} & \textit{6.0} & \textit{20.3} & \textit{9.1} & \textit{17.1} & \textit{35.2} \\ \hline\hline
         %& \textit{stdev} & \textit{17.4} & \textit{2.4} & \textit{21.6} & \textit{9.7} & \textit{6.3} & \textit{31.7} & \textit{7.5} & \textit{5.4} & \textit{3.4} & \textit{6.7} & \textit{8.3} & \textit{6.1} \\ \hline\hline
         
        \multirow{6}{*}{E} &  2 & 12.7 & 42.2 & 0.0 & 0.0 & 0.0 & 32.3 & 0.0 & 0.0 & 21.3 & 1.1 & 20.3 & 32.8 \\
         &  3 & 47.9 & 45.9 & 0.0 & 0.0 & 0.0 & 7.5 & 43.7 & 20.0 & 22.8 & 3.1 & 24.2 & 55.4 \\
         &  4 & 58.1 & 46.5 & 2.3 & 88.9 & 88.9 & 85.9 & 28.3 & 43.7 & 25.7 & 3.1 & 23.6 & 41.7 \\
         &  5 & 62.1 & 80.5 & 2.3 & 70.0 & 70.0 & 54.5 & 0.0 & 45.5 & 26.6 & 8.0 & 21.4 & 49.2 \\
         &  6 & 55.2 & 79.2 & 3.7 & 71.4 & 73.3 & 75.8 & 0.0 & 0.0 & 14.6 & 8.9 & 23.9 & 42.1 \\
         & \textit{avg} & \textit{47.2} & \textit{58.9} & \textit{1.7} & \textit{46.1} & \textit{46.4} & \textit{51.2} & \textit{14.4} & \textit{21.8} & \textit{22.2} & \textit{4.8} & \textit{22.7} & \textit{44.2} \\ \hline\hline
         %& \textit{stdev} & \textit{20.0} & \textit{19.2} & \textit{1.6} & \textit{42.7} & \textit{43.0} & \textit{32.0} & \textit{20.4} & \textit{22.3} & \textit{4.8} & \textit{3.4} & \textit{1.8} & \textit{8.5} \\ \hline\hline
         
        \multirow{6}{*}{F} &  2 & 32.7 & 69.0 & 26.0 & 0.0 & 26.0 & 27.8 & 0.0 & 0.0 & 21.7 & 2.9 & 24.5 & 49.0 \\
         &  3 & 36.7 & 74.3 & 25.4 & 31.6 & 47.1 & 7.2 & 0.0 & 1.0 & 20.0 & 0.0 & 23.4 & 47.6 \\
         &  4 & 42.4 & 68.2 & 21.6 & 22.3 & 37.9 & 72.0 & 16.3 & 2.4 & 18.0 & 1.9 & 32.0 & 45.3 \\
         &  5 & 55.9 & 73.7 & 19.8 & 88.9 & 91.3 & 40.6 & 39.6 & 0.0 & 22.2 & 6.9 & 28.6 & 47.5 \\
         &  6 & 51.7 & 74.9 & 1.6 & 31.7 & 37.0 & 100.0 & 0.0 & 45.8 & 15.0 & 0.8 & 26.8 & 44.0 \\
         & \textit{avg} & \textit{43.9} & \textit{72.0} & \textit{18.9} & \textit{34.9} & \textit{47.9} & \textit{49.5} & \textit{11.2} & \textit{9.9} & \textit{19.4} & \textit{2.5} & \textit{27.1} & \textit{46.7} \\ \hline\hline
         %& \textit{stdev} & \textit{9.8} & \textit{3.2} & \textit{10.0} & \textit{32.8} & \textit{25.4} & \textit{36.7} & \textit{17.4} & \textit{20.1} & \textit{2.9} & \textit{2.7} & \textit{3.4} & \textit{2.0} \\ \hline\hline
         
        \multirow{6}{*}{G} &  2 & 57.2 & 32.3 & 23.3 & 5.6 & 28.9 & 88.4 & 10.4 & 0.0 & 18.0 & 0.0 & 15.4 & 38.6 \\
         &  3 & 60.8 & 31.4 & 18.1 & 8.3 & 26.4 & 100.0 & 0.0 & 0.0 & 11.9 & 0.0 & 8.1 & 29.7 \\
         &  4 & 65.7 & 38.6 & 0.0 & 0.0 & 0.0 & 21.7 & 36.1 & 21.7 & 12.9 & 0.0 & 11.8 & 22.2 \\
         &  5 & 69.5 & 39.8 & 46.7 & 0.0 & 46.7 & 38.2 & 0.0 & 0.0 & 15.6 & 0.0 & 5.2 & 20.5 \\
         &  6 & 74.5 & 40.5 & 14.8 & 4.4 & 19.3 & 81.1 & 0.0 & 8.1 & 18.0 & 0.0 & 10.3 & 36.0 \\
         & \textit{avg} & \textit{65.5} & \textit{36.5} & \textit{20.6} & \textit{3.7} & \textit{24.2} & \textit{65.9} & \textit{9.3} & \textit{6.0} & \textit{15.3} & \textit{0.0} & \textit{10.2} & \textit{29.4} \\ \hline\hline
         %& \textit{stdev} & \textit{6.9} & \textit{4.3} & \textit{17.0} & \textit{3.6} & \textit{16.9} & \textit{34.0} & \textit{15.6} & \textit{9.5} & \textit{2.8} & \textit{0.0} & \textit{3.8} & \textit{8.1} \\ \hline\hline
         
        \multirow{6}{*}{H} &  2 & 11.7 & 51.5 & 4.8 & 0.0 & 53.6 & 75.9 & 0.0 & 0.0 & 13.8 & 3.1 & 17.8 & 42.6 \\
         &  3 & 30.5 & 58.7 & 60.0 & 77.8 & 92.1 & 64.4 & 25.3 & 0.0 & 25.9 & 1.0 & 10.5 & 28.0 \\
         &  4 & 30.2 & 47.0 & 58.7 & 56.1 & 79.0 & 76.4 & 0.0 & 11.5 & 27.9 & 3.4 & 18.6 & 46.1 \\
         &  5 & 32.2 & 72.8 & 62.5 & 77.8 & 86.7 & 83.7 & 0.0 & 0.0 & 24.8 & 0.8 & 20.7 & 33.9 \\
         &  6 & 33.9 & 74.6 & 50.8 & 98.2 & 98.2 & 87.7 & 24.4 & 0.0 & 26.8 & 3.1 & 21.6 & 37.9 \\
         & \textit{avg} & \textit{27.7} & \textit{60.9} & \textit{47.4} & \textit{62.0} & \textit{81.9} & \textit{77.6} & \textit{9.9} & \textit{2.3} & \textit{23.8} & \textit{2.3} & \textit{17.9} & \textit{37.7} \\\hline
         %& \textit{stdev} & \textit{9.1} & \textit{12.4} & \textit{24.2} & \textit{37.7} & \textit{17.4} & \textit{8.9} & \textit{13.6} & \textit{5.1} & \textit{5.7} & \textit{1.3} & \textit{4.4} & \textit{7.1}
        
    \end{tabular*}
\end{table*}

% \subsection{Correlation of Testing Metrics and Functional Suitability}

% Based on the statistical modelling we can see that direct correlation between percentage of overall test coverage and percentage of passed stories per sprint (functional suitability). 
% This trend is particularly obvious for Teams C and Team H . Figures~\ref{fig:team-c} and \ref{fig:team-h} visually show the improvement in testing coverage together with the assessment of the functional suitability.

% Team C started with reasonable level of backend unit test coverage but very low acceptance testing, hence functional suitability, (product quality) is only ~40\% of story points. The product quality has increased to over 70\% and has continued to increase in sprint 6 reaching the total of 100\% success rate. This seems to be related to the increase of automated acceptance testing and manual testing in sprint 4 \& 5. During sprint 6 most teams focus on testing and/or fixing (see Table 2) as this is their last sprint and product was to be prepared for the final presentation to the wider audience (the department and industry). Therefore, it is not surprise that most of the teams have improved the product quality in the last sprint.

% Team H had reasonable level of backend and acceptance testing right through the project and consequently the functional suitability was stable throughout the year (on ~80\% on average).

% The exception to this trend can be observed in Team F. The team has had continuously high back-end unit testing but low front-end unit testing and acceptance testing throughout the year. Their functional suitability has been very unstable. The fluctuation in product quality was going in the opposite direction to the acceptance testing trend (e.g. when manual testing was at its pick in sprint 5, the functional suitability dropped significantly). This required inspection of additional influencing factors. 

% Team F seems to have performed better when the sprint was including a break (term or semester break). When a sprint was worked on during term time only, they seem to have struggled to produce a high product quality (sprint 3 \& 5). This could be related to the fact that this was a team of high performing individuals who worked hard on other courses during a term and therefore they focused on the project course more over the break, as there was a bit of flexibility to do so. Therefore the code quality and testing effort seem to have improved during these sprints (sprint 4 \& 6).

% Also, in sprint 5 manual acceptance testing significantly improved (2.5 x increase from previous sprint), but the functional suitability didn't follow. This was curious so we looked further.
% %and we looked at the manual testing coverage on AC level. Looking at the manual tests produced we noticed that they tried to increase the coverage by having only 1 manual test for each AC. Even though we assume that AC is covered if there is at least on manual test written for it, this often is not enough, and having such light coverage does not guarantee functional suitability for every AC.

% We noticed that in sprint 5 Team F had a very optimistic sprint estimate/commitment which lead to huge deferral ( 40\% of story points, see DSP, Table ~\ref {tbl:team-metrics}). The team had to spend some time on these stories but the effort didn't pay off as they decided to defer. This effort doesn't contribute to current sprint outcome but does increase success rate of the next sprint as students have already put some thoughts into those stories (and potentially wrote some code for it). Based on the difference between passed story and passed story points percentage, we can conclude that they have passed simpler stories and stories that failed in the previous sprint but that they have failed and deferred more complex ones, new/unfamiliar stories.
% In sprint 6, they reached very high level of functional suitability even though the testing effort appeared to have dropped (see Figure 7, sprint 6). In this sprint they have 46\% of redeemed story points suggesting that half of the backlog was made out of deferred and failed stories from previous sprint. These are the stories that they worked on before and were easier to get right due to their previously acquired knowledge. At this stage the testing seems to have been mostly on the development level, therefore not always logged.




% - Should I be looking at the following data where we are observing lack of product quality while testing was high :
%     - Team dynamics
%     - sicknesses
%     - other course work and lack of planning of their time
%     - over committing and lack of planning
%     - not enough experience with automated acceptance testing (high testing \% in that case doesn't necessary average the high product quality)
%     - ?

% Some of the possible reasons why teams did well in-spite of the low testing stats:
% - gained experience in technology they were using over time, so less problems introduced 
% - working on fixes not complex new implementation
% - change of marker? 

% - Is it worth adding a bit of maths to this by seeing what is the standard deviation for correlation between high testing and high quality, or is the sample of data too small to look into this.

%  Team-G presented another example of inconsistent testing and quality. This team has invested in front-end testing mostly (unit testing for Jest) while back-end and automated acceptance testing was on the average to low level. Manual testing was almost non-existable and automated acceptance testing was done but inconsistently. This suggests that testing strategy focused on front-end testing only does not result in desirable product quality. This conclusion is supported by comparing this team to Team-H were front-end testing was low but the overall product quality was high, due to high level of coverage in back-end, automated acceptance testing and manual testing. 

% Team E has had somewhat similar pattern to Team F. They have deferred 44\%  of stories in sprint 3 and have then worked on these stories in sprint 4. This previously acquired knowledge would have given them a significant advantage when working on these stories. They also significantly increased their manual testing coverage in sprint 4. Those two factors seem to have had a combined effect on their success rate in sprint 4 (~80\%).

% In sprint 5 they have deferred 28\% of story points. By looking at the passing story points rate (lower than a story passing rate) they seem to have focused on easier stories and deferred more complex ones. This kept they product quality on reasonably high level of ~80\%. By looking at the graph for Team-E, sprint 5, manual acceptance testing coverage seems lower then in sprint 4, even though they have spent more hours manual testing (~25h in sprint 5, compared to ~12h in sprint 4). This is a bit miss-leading as they seem to have written (and executed) more tests per story in sprint 5. They have had 53 manual tests over 4 stories compared to 50 manual tests over 9 stories in sprint 4. So, the manual testing effort was still very high (even though not quite reflected through the coverage)  which seemed to has keep the product quality at high level. We can observe the similar behaviour in sprint 6.

% Team D was the team that if we were to look at the overall testing coverage and story passing rate it would appear that testing didn't directly made any difference to their success rate (especially in sprint 3 and 4). For example, in sprint 4, the team had low product quality (35\% of story points passed), while overall acceptance testing was on a reasonable level (71\%). When inspecting the acceptance testing on individual story level (more granular data not available in the paper) we could see that they had very low number of acceptance tests per AC (often only 1) , but as we (for practical reasons) assume that AC is covered if there is at least one acceptance test (automated or manual ) implemented, we have considered these stories fully tested. For some ACs one test per AC does not cover all potential scenarios covered in an AC, and quite a few stories failed as a result. 
% % do we want to mention that having one manual test per AC might be a problem, as it might affect the validity of our initial assumtion

% In sprint 5, even though overall acceptance testing dropped to 50\%, they have passed all stories. Again, this required a closer inspection of the sprint commitment and acceptance testing records. In this sprint, 6/10 stories worked on, were failed stories from previous sprint. So only small fixes have been required. The team knew exactly what needs fixing based on the feedback they got from the teaching team. These stories didn't have high level of acceptance testing but as only minor fixes were required, there was less of a chance that something would go wrong. Other 4 (new) stories have been fully acceptance tested and therefore passed the review. So, this team success rate still very much depended on the level of testing they have done.
% Team A has failed large portion of their stories in the first 3 sprints and have put many hours towards fixing their issues in sprint 4. They also improved in all aspects of testing from sprint 4 onwards. This is the sprint where we have seen the first significant improvement in the product quality. The fact that they deferred 1/5 of their commitment in this sprint also helped with success rate (if they haven't deferred, they would have most likely failed them). In sprint 5 \& 6 they further increased FEUT, BEUT AAT (in sprint 5 only) and MAT. We could see significant improvement in PSP in these two sprints too.

% Team B has not been very consistent with the way they have been recording their acceptance testing (manual testing mostly). Often it was hard to determine a match between a test and an AC.  This has resulted in somewhat inconclusive picture. In sprint 2 \& 3 they had very low unit test coverage (below 40\%) , same goes for acceptance test coverage. It is therefore not a surprise to see that their PSP was very low too (14.5\% and 0\% respectively )  They have had a high deferral rate in sprints 2 \& 3 \& 4 and consequently high redeemed story points rate in 3 \& 4 \& 5, which suggests that they had trouble estimating and planning sprint commitment in those sprints.  In sprint 4 they have managed to pass over 50\% of story points even though their manual testing and automated acceptance testing dropped significantly. Which could be due to the high redeemed story points rate (worked on the stories they have failed in previous sprints). They have also continuously increased their front-end and have had a close to full coverage of manual acceptance testing in sprint 5 resulting. This improvement in FEUT and MAT followed by the improvement in PSP goes in line with previously found correlation between front-end unit testing and functional suitability. 

% In sprint 6, team didn't have any manual or automated acceptance testing, while both front-end and back-end unit testing has increased only by a little (~10\% increase) but have still managed to reach a highest level of PSP (83\%). They worked on 4 new, good size stories (8-13 points), so didn't have any redeemed story points in their commitment, but yet managed to do well. This confirms that increase in FEUT is making a significant impact to product quality (as fund in statistical analysis)

%Team-A has spent many hours on testing but not much on manual testing while they still have some manual tetsing coverage. I wonder if they logged it all under test tag. For example in sprint 5 they have had 31 tests but have spent only 0.6h on manual testing. Is this even possible to do?

% Do we need this now???
% The pattern of teams work distribution over time is another important aspect of team work and their impact on overall product quality (functional suitability). To get this overview we have look at summary of time teams spent on specific tasks per sprint. We have collected the worklog data and calculated  the percentage of total logged time spent on fixes, testing (automated and manual) and implementation. We have looked for correlation between the portion of time spent on testing and the actual test coverage as well as if there is consequential increase in hours spent on fixes followed by a poor deliverable.  
% As discussed in Data Sources section, students have used project management tool \textit{Jira}\footnote{See \url{https://www.atlassian.com/software/jira}} to classify and log time spent on the project. The tags we are mostly interested here are those related to implementation, testing (automated and manual) and fixes (see Table 1).   

% % do we need this paragraph we have covered this laready elsewhere

% It is worth noting that, often students would use more than one tag to record the time spent in a session. For example, when they work on a new feature but also write unit tests in the process, they would log their total time spent using \#implementation and \#test tag. The total time logged would have been added to both tag summaries (e.g. a 3h session with tags \#implementation and \#test would have increased both tags total for that sprint for 3h hours).  Therefore this metric should be used to determine a trend of work distribution for teams over the time rather than an absolute (accurate) value of total time spent on the project. 

% Team F: 
% By looking at the hours they spent on various activities (see Table 2) we can notice that they spent many hours fixing issues from sprint 3 (the sprint with lowest product quality) in sprint 4. This resulted in second highest number of hours spend on fixes any team had for the duration of the year - 154.4h ( see Table 2). Similar thing happened in sprint 6 for Team F, number of hours spent on fixing increased after an unsuccessful sprint 5 (just over 40\% of passed stories).
% Team F also seem to have had a problem with planning and estimation even later in the year. They were the team of strong, overconfident individuals which put the high expectations on themselves.   More specifically in sprint 3 they passed only 7\% of story point (see SP column in Table 1). In sprint 4 they seem to have spent a lot of time fixing the sprint 3  issues (see Table 2, fix tag for sprint 4)  
% The product quality for sprint 4 appears to be much higher than in sprint 3. Testing and fixing effort has increased (Table 2) .

% In sprint 6 team has reduced an overall testing effort, while fixes and new features implementation hours have increased. This is another example of drop in product quality sprint (sprint 5) followed by a sprint with increased fixing effort.  As this was the last sprint spent a lot of time fixing the product and preparing for the final delivery. This seem to have helped the team reach high product quality.
% Overall, this team did better when they have spent more time fixing issues (not necessary testing). The way the fixing has been done here could be associated with white box testing, when a developer examines the written code and subsequently test locally made changes (bug fixes). It is obvious that they would have benefited from more thorough overall acceptance testing during the sprint.

% Team E spent many hours fixing issues from sprint 3 which, as we have seen with Team-F, often boosts the passing rate (small code changes followed by manual testing). Overall manual testing effort has increased significantly in sprint 4 which improved overall acceptance testing coverage and subsequently the product quality (to 86\% passing story points in sprint 4). 

% Team A -This team seem to have logged all their testing hours under the test tag, as we can see the effort put towards testing from sprint 4 onwards has significantly increased. They seem to have logged most of their manual testing under this tag too, as effort logged under manual testing tag does not matched the number of test written and run. For example, in sprint 5 they have had 31 manual tests in total but have only logged 0.6h under manual testing.
% %


%Discuss handling of mortality
%Discuss the fact that markers are changing from sprint to sprint so there is some subjectivity when marking.
% Must talk about MAT being acceptance testing-driven

%\subsubsection{Validity procedure}

%cite ~\cite{Runeson2012}
